Generalisable Methods for Early Prediction in Interactive Simulations for Education

Interactive simulations allow students to discover the underlying principles of a scientific phenomenon through their own exploration. Unfortunately, students often struggle to learn effectively in these environments. Classifying students' interaction data in the simulations based on their expected performance has the potential to enable adaptive guidance and consequently improve students' learning. Previous research in this field has mainly focused on a-posteriori analyses or investigations limited to one specific predictive model and simulation. In this paper, we investigate the quality and generalisability of models for an early prediction of conceptual understanding based on clickstream data of students across interactive simulations. We first measure the students' conceptual understanding through their in-task performance. Then, we suggest a novel type of features that, starting from clickstream data, encodes both the state of the simulation and the action performed by the student. We finally propose to feed these features into GRU-based models, with and without attention, for prediction. Experiments on two different simulations and with two different populations show that our proposed models outperform shallow learning baselines and better generalise to different learning environments and populations. The inclusion of attention into the model increases interpretability in terms of effective inquiry. The source code is available on Github (https://github.com/epfl-ml4ed/beerslaw-lab.git).

==> [EDM 2022] Generalizable Methods for Early Predictions in Interactive Simulations (Copy)/context.tex <==
\section{Learning Environments}\label{section:contextdata}
%\section{Learning environments}
% Describe chemlab + capacitor (shorter)
% Does the paper provide detail on the demographics of the population involved in the study?
% Does the paper describe how participants’ privacy rights were respected in the data collection process?
The PhET interactive simulations\footnote{https://phet.colorado.edu/} allow students to explore natural phenomena using different parameter configurations and ideally infer the underlying principles on their own. A large body of research has focused on analysing students' inquiry strategies using these simulations, usually coupled with an explicit task to be solved using the simulation \cite{yehya2019learning}. To evaluate the (early) prediction models presented in this paper, we used a ranking task which we adapted to two different simulation environments. \jade{For each ranking task, the values of the variables presented in the task are outside the range provided by the simulation. Hence, students need to inquire the system to uncover the appropriate equations and plug in the numbers as answers in the ranking task.}
% To be able to solve the ranking task, students need to infer the principles governing the simulation.
%The methods presented in this paper were evaluated with two data sets collected from classroom experiments in which students solved inquiry-based learning tasks using two of the PhET interactive simulations\footnote{https://phet.colorado.edu/}. While different simulations were used for each data set, the associated learning tasks were designed in a similar way thus enabling the application of the same analysis methods for both data sets.

\begin{figure} 
\Description{The two learning environments used to collect both datasets in this paper are depicted: the capacitor lab on the left, and the beer's law lab on the right.} 
\centering \includegraphics[width=\columnwidth]{EDM-template/figures/Fig_phet_envs.JPG} \caption{The two learning environments used in this study, the Capacitor Lab (A) and the Beer's Law Lab (B).} 
\label{fig:phet-envs} 
\end{figure}

\begin{figure}[!t]
\Description{TODO}  % Alt text
\centering
\subfloat[Task for the Capacitor Lab simulation \cite{cock2021early}. ]{\includegraphics[width=\columnwidth]{EDM-template/figures/caplab_task.png}}\\
\subfloat[Task for the Beer's Law Lab simulation. ]{\includegraphics[width=\columnwidth]{EDM-template/figures/fig_ranking_beer.pdf}}\label{fig:ranktaskchemlab}
\caption{Ranking tasks for the two interactive simulations.}
\label{fig:ranktask}
\end{figure}

\textbf{Capacitor Lab}. The PhET Capacitor Lab simulation\footnote{https://phet.colorado.edu/en/simulations/capacitor-lab} provides students with the possibility to manipulate different parameters of an electric circuit (plate area, plate separation, applied voltage, open/close the circuit), to help them understand how each parameter influences the capacitance of a plate capacitor as well as the energy stored in that capacitor (see Fig. \ref{fig:phet-envs}A). Previous work \cite{cock2021early} designed an inquiry-based learning activity for this simulation using a ranking task. Specifically, students were asked to rank four different configurations according to the stored energy saved in the plate capacitor (see Fig. \ref{fig:ranktask}a). The four configurations were created by first loading the plate capacitor using two parameter configurations in a closed circuit (A and B), followed by opening the switch to disconnect the capacitor from the circuit and changing the parameters to obtain the final configurations to be ranked (1, 2, 3, and 4). The authors also suggested a tree-based approach to label the $24$ possible solutions based on conceptual understanding. For this paper, we will use the binary labels suggested by \cite{cock2021early} to divide students into a group with an \texttt{advanced understanding} of stored energy (i.e., for both open and closed circuits) and a second group with a conceptual understanding limited to the closed circuit, denoted as \texttt{limited understanding}.

\textbf{Beer's Law Lab}. The PhET Beer's Law Lab simulation\footnote{https://phet.colorado.edu/en/simulations/beers-law-lab} allows students to explore how light is absorbed in a solution and which factors influence the measured absorbance (Fig. \ref{fig:phet-envs}B). In this environment, the students can manipulate the following components: the wavelength $\lambda$ of the light beam, the width of the container (representing the light's path length $L$ through the solution), the substance of the solution (changing its colour), and its concentration $c$. By experimenting with these components, in the ideal case, students can infer Beer's Law, which describes how each parameter influences the measured absorbance: $ A = \epsilon_\lambda * L * c $. Based on the inquiry-based learning task presented by \cite{cock2021early}, we developed a ranking task that can be solved with Beer's Law Lab. Students were presented with four flasks that varied in width as well as in the color and concentration of the solution they contained (Fig. \ref{fig:ranktask}b). Given a light beam of a specific wavelength, students were asked to rank the four flasks by the measured absorbance. It is important to note that the values chosen for the four flasks were not available in the simulation in order to prevent students from obtaining the correct ranking by simply replicating the flasks. To label the submitted rankings, we used the tree-based approach introduced in previous work \cite{cock2021early}. We classified each of the $24$ possible rankings according to the level of conceptual understanding (Fig. \ref{fig:labelschemlab}). Specifically, for each ranking, it was determined whether the influence of i) the substance's concentration, ii) the container's width and iii) the colour difference between light beam and solution was understood or not. Rankings were then grouped by the number of concepts understood that they represented. Rankings representing $0$ or $1$ concepts understood were then labelled as \texttt{limited understanding}, while rankings representing $2$ or $3$ concepts were labelled as \texttt{advanced understanding}.

\begin{figure}[t]
\Description{TODO}  % Alt text
\centering
\includegraphics[width=\columnwidth]{EDM-template/figures/fig_labels_beer.pdf}
\caption{The tree used to map the rankings to different levels of conceptual understanding. The numbers in parentheses indicate the number of submissions for the ranking.}
\label{fig:labelschemlab}
\end{figure}

%\begin{figure}
%\Description{Four flasks: 1) green solution, width of 3 cm, concentraion of $5microMol/L$, 2) green solution, width of 3cm, concentraion of 200micro mol per liter, 3) red solution, width of 4.5 cm, concentration of 150 micro mol per liter. 4) red solution, width of 0.75cm, concentration of 250 micro mol per liter.}  % Alt text
%\centering
%\includegraphics[width=\columnwidth]{EDM-template/figures/fig_ranking_labels.pdf}
%\caption{A) The ranking task presented for the Beer's Law Lab. B) The tree used to map the rankings to different levels of conceptual understanding. The numbers in parentheses indicate the number of submissions for the ranking. }
%\label{fig:ranking-task-chemlab}
%\end{figure}


%All experiments described in this paper are conducted with interaction logs generated by the PhET interface. Those were collected during user studies in which we evaluated students' inquiry and problem solving skills. In the rest of this section, we describe the learning activities, pre-processing of the interaction logs, features extractions and model architectures implemented to classify students according to their conceptual understanding of different scientific topics.

%\textbf{Capacitor Lab Activity.} To assess the generalizability of the presented methods, a second data set was used in the analyses. This data was collected in a previous work \cite{cock2021early} involving experiments with the Capacitor Lab simulation. This environment provides students with the possibility to manipulate different parameters of an electric circuit (plate area, plate separation, applied voltage, open/close the circuit) to help them understand how each of them influences the energy stored by a plate capacitor (Fig. \ref{fig:phet-envs}B). Analogously to the Beer's Law Lab activity, a ranking task was designed and presented to the students. In this case, students had to rank four different configurations of plate capacitors by the energy they stored. Using the same tree-based approach, the submitted rankings were then labeled and classified into two main groups: the first group included all the rankings representing a complete understanding (i.e., both open and closed circuits), whereas rankings in the second group represented an understanding limited to the closed circuit. For more details on the design of the ranking task as well as the labeling procedure, please refer to the original work \cite{cock2021early}.

==> [EDM 2022] Generalizable Methods for Early Predictions in Interactive Simulations (Copy)/method.tex <==
\section{Method}
\label{sec:method}
We are interested in creating \textit{generalisable models} to (early) predict the level of conceptual understanding students will achieve after interacting with a simulation. Formally, our goal is to predict, for each student, a binary label representing their level of conceptual understanding. To address this binary classification task, we propose a pipeline consisting of the four steps illustrated in Fig. \ref{fig:datapipeline}. We first pre-process the data into event logs and extract so-called state-action sequences from these event logs. We then build different types of deep neural network models to perform the classification task. In what follows, we first formalise the addressed problem, before describing each step of the pipeline in detail.

\begin{figure*}[t]
\Description{The data pipeline consist in 1) the data processing (states and actions are combined, and the shortest 60\% breaks are discarded as being non relevant to the user interaction), 2) The feature extraction part (states and actions are categorised into a small number of groups), 3) model building (the data is fed into a GRU and an attention GRU to (early) predict students' conceptual understanding).}  % Alt text
\centering
\includegraphics[trim= 0.0 0.0 0cm 4.5cm,width=0.8\textwidth]{EDM-template/figures/methodspipeline.pdf}
\caption{Our model building pipeline consists of three steps: we first extract the logs into sequences of events and states. We then categorise the states and events to build state-action sequences. Finally we feed the features into variations of GRU models.}
\label{fig:datapipeline}
\end{figure*}

\begin{figure*}[!t]
\Description{Architecture of our GRU model with one unrolled GRU layer: the input time steps are fed sequentially into the recurrent cells of the GRU layer. The output of the last GRU cell is fed to the dense layer which is then SoftMax activated to determine the probability of the student belonging to each of the 2 classes.}  % Alt text
\centering
\includegraphics[trim= 0.0 0.0 0cm 4.5cm, clip,width=0.7\textwidth]{EDM-template/figures/GRUDL.pdf}
%   \includesvg[width=\columnwidth]{figures/GRUDL.svg}
\caption{Architecture of our \texttt{GRU} model with one unrolled GRU layer: the input features are fed sequentially into the recurrent cells of the GRU layer. The output shape of each layer is given: $|U|$ denotes the number of users, $\tilde{n} = \max_{u\in\mathcal{U}} \tilde{n}_u$, $cell$ the number of GRU cells, and $f$ the number of features in the input matrix.}
\label{fig:grudl}
\end{figure*}


\subsection{Problem Formalisation}
We consider $\mathcal{U}$ to be the set of students participating in the learning activity. During this learning activity, students use an interactive simulation in order to rank four different configurations according to a specific criterion (see Section \ref{section:contextdata} for details on the ranking tasks). We denote the set of possible answers to the ranking task as $\mathcal{A}$ and the answer of a student $u \in \mathcal{U}$ to this ranking task $a_u \in \mathcal{A}$. Based on their answers, we assign a label $L_u \in \{0, 1\}$ to each student $u \in \mathcal{U}$. This mapping $m$ is a direct function of students' answers and can be formalised as  $m: a_u\in \mathcal{A} \longmapsto L_u \in \{0, 1\}$ for $u\in \mathcal{U}$. For both lab activities, label $1$ denotes \texttt{advanced understanding} and label $0$ \texttt{limited understanding}.

\par To solve the ranking task, students interact with the simulation and investigate the factors influencing the dependent variable (absorbance in case of Beer's Law Lab, stored energy in case of Capacitor Lab). Their full and non-processed sequence of events in the simulation is denoted as:
\vspace{-5mm}

\begin{equation}\label{eq:rawsequence}
    R_u = \{(e_0, s_0, d_0), ..., (e_{n_u-1}, s_{n_u-1}, d_{n_u-1})\}
\vspace{-2mm}
\end{equation}

where $e_m$ is the $m^{th}$ \textit{event} $e$ , $s_m$ is the \textit{state of the simulation} at time step $m$, and $d_m$ denotes the \textit{duration of event} $e_m$ in \textit{state} $s_m$.
We denote the partial sequence of student $u \in\mathcal{U}$ from the first to the $l^{th}$ event as $R_u^l=\{(e_0, s_0, d_0), ..., (e_{l-1}, s_{l-1}, d_{l-1})\}$ with the value $l\in[1, n_u)$.
To clarify the notion of \textit{duration} and \textit{time steps}, we introduce $\|R_u\|_{duration} = t_u$ where $t_u$ denotes the total time in seconds spent by student $u$ on the simulation. We then denote $\|R_u\|_{timestep} = n_u$ where $n_u$ denotes the total number of events performed by student $u$ in sequence $R_u$.

Hence, training an (early) students' conceptual understanding predictor $\mathcal{E}$ with interactions $R_u$ and conceptual label $L_u$ after a number of interactions $\bf{n}_u$ becomes an optimisation problem, aimed to find model parameters $\theta$ that maximise the expectation on the following objective function (i.e., predict the correct label, given interactions) over a dataset $\mathbb G$:
\vspace{-10mm}

\begin{equation}
\tilde{\theta} = \underset{\theta}{\operatorname{argmax}} \mathop{\mathbb{E}}_{(R_u, L_u)\in \mathbb{G}}  L_u = \mathcal{E}(R_u^{\bf{n}_u} \;|\; \theta)
\label{eq:problem-definition}
\vspace{-2mm}
\end{equation}

In what follows, we describe the steps carried out to solve this problem from pre-processing until model building.  

\subsection{Data Pre-Processing}
From the log data, we extract the sequence of events of a student $u$ as follows: anything between a mouse click and a mouse release qualifies as an \textit{action}. Each \textit{action} can be described by its \textit{duration} and the \textit{component} the action is performed on, and is conducted in a specific \textit{simulation state}. Anything between a mouse release and a mouse click qualifies as a \textit{break}. Similarly, \textit{breaks} are conducted in a specific \textit{state} and have a specific \textit{duration}.
All \textit{actions} and \textit{breaks} generated by a student $u\in\mathcal{U}$ are sorted chronologically to form the raw interaction sequence of a user $u\in\mathcal{U}$, $R_u$ as per Eq. \ref{eq:rawsequence}, where events can be both \textit{actions} or \textit{breaks}.

Some \textit{breaks} in student interactions can be indicative of reflective, observational or distracted periods. Other \textit{breaks} can occur naturally throughout a student's interaction when the mouse moves from one element to the other \cite{wang2021examining}. The latter might introduce undesired noise and hinder student classification over their conceptual understanding, not unlike stop words negatively influence sentiment analysis tasks in the domain of natural language processing, as an example \cite{ghag2015comparative}. To maximise the retention of informative periods of inactivity, we therefore discard for each student $u\in\mathcal{U}$ their $60\%$ of shortest breaks. We are left with $R_u = \{(e_0, s_0, d_0), ..., (e_{\Tilde{n}_u-1}, s_{\Tilde{n}_u-1}, d_{\Tilde{n}_u-1})\}$ with $\Tilde{n}_u \leq n_u$, the final sequence of triplets of events $e_m$ occurring in state $s_m$ and of duration $d_m$ for student $u\in\mathcal{U}$ at time $m\in[0, t_u)$. \jade{The new sequence contains $\tilde{n}_u$} event triplets, i.e., \textit{timesteps}.

\begin{figure*}[!t]
\Description{\texttt{SA-GRU} architecture with the depiction of the attention mechanism for timestep $t$.}  % Alt text
\centering
\includegraphics[width=0.86\textwidth]{EDM-template/figures/SAGRU.pdf}
%   \includesvg[width=\columnwidth]{figures/SAGRUDL.svg}
\caption{\texttt{SA-GRU}'s architecture with the attention mechanism. The output shape of each layer is given: $|U|$ denotes the number of students, $\tilde{n} = \max_{u\in\mathcal{U}} \tilde{n}_u$, $f$ is the number of dimension in the state-action features, and $cells$ is the number of GRU cells.}
\label{fig:sagrudl}
\end{figure*}

\subsection{Feature Extraction}
\label{sec:featextract}
% Be more general -> state of the siulation + for chemlab it would look like that, and for capacitor lab it would look like that
\jade{The data logging of the PhET environments captures any click targeting an "interactive" component as well as the state of the simulation in case one of these "clicks" changes the value of a variable/multiple variables in the system. This fine-grained logging results in high dimensional simulation states $s$ and a high number of different events $e$. Before creating feature vectors for each time step $m$, we therefore categorise the obtained events and states into meaningful components. We divide all possible \textit{simulation states} into two groups: a) helpful or b) unhelpful to solve the problem. We then ponder whether some of the \textit{helpful states} can be grouped such that the level of information received by the student is the same independent of the state within the group. We proceed in a similar way for the events. While this categorisation procedure is generalisable over different platforms, whether a simulation state or event is helpful depends on the actual task.}

\jade{\textbf{State-Action Categorisation for Capacitor Lab}. For the Capacitor Lab activity, we use the state and action categorisation defined in \cite{cock2021early}. By applying the above pipeline, we qualify each state $s_m \in (e_m, s_m, d_m)$ into one of the following groups: 1) closed circuit - stored energy displayed, 2) open circuit - stored energy displayed, 3) closed circuit - stored energy not displayed, and 4) open circuit - stored energy not displayed. Since stored energy is the dependent variable in the ranking task, displaying the stored energy is essential for solving the task. The relationship between the parameters (plate area, plate separation, battery voltage) and stored energy differs for closed and open circuits. Moreover, we map each event $e_m \in (e_m, s_m, d_m)$ into one of the following actions: 1) manipulating battery voltage, 2) manipulating plate area, 3) manipulating plate separation, 4) break, 5) other (any other action). }

% \textbf{State-Action Categorisation for Capacitor Lab}. For the Capacitor Lab activity, we use the state and action categorisation defined in \cite{cock2021early}. Consequently, we categorise each state $s_m \in (e_m, s_m, d_m)$ into one of the following four groups: 1) closed circuit - stored energy displayed, 2) open circuit - stored energy displayed, 3) closed circuit - stored energy not displayed, and 4) open circuit - stored energy not displayed. Since stored energy is the dependent variable in the ranking task, displaying the stored energy is essential for solving the task. The relationship between the different parameters (plate area, plate separation, battery voltage) and stored energy differs for closed and open circuits. Moreover, we map each event $e_m \in (e_m, s_m, d_m)$ into one of the following actions: 1) manipulating battery voltage, 2) manipulating plate area, 3) manipulating plate separation, 4) break, 5) other (any other action). 

\vspace{-1mm}
\jade{\textbf{State-Action Categorisation for Beer's Law Lab}. There are four independent variables that influence the dependent variable \textit{absorbance} of the ranking task: the \textit{laser colour}, the \textit{solution colour}, the \textit{concentration} of the solution, and finally the \textit{width} of the container. Consequently, we categorise each state $s_m \in (e_m, s_m, d_m)$ into one of those 4 groups: 1) green-green (absorbance: displayed, laser colour: green, solution colour: green), 2) green-red (absorbance: displayed, laser colour: green, solution colour: red), 3) absorbance displayed (absorbance: displayed, laser colour: not green and/or solution colour: neither red nor green), 4) not observed (absorbance: not displayed). To solve the ranking task depicted in Fig. \ref{fig:ranktaskchemlab}, students need to understand how the \textit{width} and \textit{concentration} interact with the \textit{absorbance} when the \textit{solution colour} is either red or green and when the \textit{laser colour} is green, i.e., states 1) and 2). The \textit{width} and the \textit{concentration} share a linear dependency with the \textit{absorbance} and are both colour agnostic. As long as the absorbance is observed, those relations can be discovered no matter the colour of the laser or the solution, i.e., state 3. Furthermore, we process each event $e_m \in (e_m, s_m, d_m)$ into one of those categories: 1) width (width slider is moved), 2) concentration (concentration slider is moved), 3) pdf (students are reading the instructions from the ranking task), 4) concentration lab (students are interacting with the second simulation available directly from the Beer's law lab), 5) breaks, 6) other.}

% \textbf{State-Action Categorisation for Beer's Law Lab}. There are four independent variables that influence the dependent variable \textit{absorbance} of the ranking task: the \textit{laser colour}, the \textit{solution colour}, the \textit{concentration} of the solution, and finally the \textit{width} of the container. Consequently, we categorise each state $s_m \in (e_m, s_m, d_m)$ into one of those 4 groups: 1) green-green (absorbance: displayed, laser colour: green, solution colour: green), 2) green-red (absorbance: displayed, laser colour: green, solution colour: red), 3) absorbance displayed (absorbance: displayed, laser colour: not green and/or solution colour: neither red nor green), 4) not observed (absorbance: not displayed). To solve the ranking task depicted in Fig. \ref{fig:ranktaskchemlab}, students need to understand how the \textit{width} and \textit{concentration} interact with the \textit{absorbance} when the \textit{solution colour} is either red or green and when the \textit{laser colour} is green, i.e., states 1) and 2). The \textit{width} and the \textit{concentration} share a linear dependency with the \textit{absorbance} and are both colour agnostic. Consequently, as long as the absorbance is observed, those relations can be discovered no matter the colour of the laser or the solution, i.e., state 3. Furthermore, we process each event $e_m \in (e_m, s_m, d_m)$ into one of those categories: 1) width (width slider is moved), 2) concentration (concentration slider is moved), 3) pdf (students are reading the instructions from the ranking task), 4) concentration lab (students are interacting with the second simulation available directly from the Beer's law lab), 5) breaks, 6) other (any other actions including those related to the laser's colour and the solution's colour as both are implicitly included in the state encoding).

\textbf{State-Action Sequences}. After the categorisation step, each $e_m \in (e_m, s_m, d_m)$ will have been replaced by $e_m'$, its corresponding event category, and each $s_m \in (e_m, s_m, d_m)$ will have been replaced by $s_m'$, its corresponding state mapping. For each timestep $m$, we encode $s'_m$ as a one-hot-encoded vector $v^{s'}_m$ of $c_s$ cells (with $c_s$ denoting the number of different state categories for the simulation), where all entries are $0$ except the one corresponding to $s'_m$, which is equal to $1$. We also transform $e'_m\in(e'_m, s'_m, d_m)$ into a one-hot-encoded vector $v^{e'}_m$ of $c_e$ cells (with $c_e$ denoting the number of different event categories for the simulation), where all entries are $0$ except the one corresponding to $e'_m$, which is equal to $d_m$. Finally, for each time step $m$, we replace each triplet $(e'_m, s'_m, d_m)$ by the concatenation of both vectors $v^{s'}_m$ and $v^{e'}_m$. 
For each student $u\in\mathcal{U}$, the interaction sequence $R_u$ can now be formulated as $\{[v^{s'}_0, v^{e'}_0], ..., [v^{s'}_{t_u-1}, v^{e'}_{t_u-1}]\}$.
We then normalise the sequences on the $v^{e'}_0$ dimension resulting in the final action sequence $F^{SA}_u$ for student $u\in\mathcal{U}$.

\vspace{0mm}
\subsection{Model Building}
In this paper, we are interested in creating a conceptual understanding prediction model that can accurately predict the conceptual understanding label $L_u$ for student $u$, given the extracted features $F_u^{SA}$. To this end, we rely on two types of models, both based on a \textit{Gated Recurrent Unit} (GRU) network \cite{cho2014properties}. GRUs are a type of Recurrent Neural Networks (RNNs), whose specificity is to allow the transmission of information over time. To process sequential data, RNNs are composed of $r$ recurrent cells arranged successively such that the output of one becomes the input of the next one, as illustrated on Figure~\ref{fig:grudl}. Their relative simplicity enables GRUs to handle smaller datasets (as those in our hands) than the more complex long short-term memory cells (LSTM), which contain an additional output gate~\cite{lstmchung2014empirical, lstmgruber2020gru}.

The first type of model is based on a GRU combined with a Dense layer (\texttt{GRU}), as shown in Figure \ref{fig:grudl}. Specifically, the extracted features $F^{SA}$ are fed into a neural architecture composed of a \emph{GRU}, a \emph{dropout} layer and a \emph{Dense} layer (with Softmax activation) having a hidden size of $1$. The model outputs the probability the student $u$ will gain advanced (label $1$) or limited (label $0$) understanding.

The second type of model is based on a Self-Attention-based Gated-Recurrent-Unit (\texttt{SA-GRU}), as shown in Figure \ref{fig:sagrudl}. In 2014, the concept of an \textit{Additive Attention} layer, also called \textit{Bahdanau attention} was introduced to improve statistical machine translation \cite{bahdanau2014neural}. Rather than using it to understand the context of words across languages, we use it to identify the pivotal moments in students' interactions with the simulation. We first take the raw extracted features $F^{SA}$ as the \textit{query}, \textit{key} and \textit{value} input matrices to our self-attention mechanism implemented as in \cite{attentionimplementation}. We then concatenate the attention output with the input features along each time step and feed this matrix to a GRU layer. Its latest output will directly be given to the dropout layer before passing through the final Dense layer which uses a Softmax activation (analogously to the \texttt{GRU} model). Though more complex than \texttt{GRU} and consequently more subject to overfitting on smaller datasets, \texttt{SA-GRU}'s attention weights can be used to understand what dimension of our features are important for the final prediction, and when that importance is emphasised over time. These aspects are fundamental to enable interpretability on such complex yet effective models. 


==> [EDM 2022] Generalizable Methods for Early Predictions in Interactive Simulations (Copy)/results.tex <==
\section{Experimental Evaluation}
\label{sec:results}
We evaluated our (early) prediction models on two data sets collected using the ranking task activities on the PhET Beer's Law Lab and Capacitor Lab simulations (see Section \ref{section:contextdata}). We used the data set that we collected using the Beer's Law Lab activity as an \textit{evaluation data set} to assess to what degree student interaction data within the simulation is predictive for their obtained conceptual understanding (RQ1) and whether our models are able to predict students' conceptual understanding at the end of the task \textit{early} on (RQ2). We then used the data that was collected by previous work \cite{cock2021early} using the Capacitor Lab activity as a \textit{validation data set} to assess the transferability of our proposed models to a different population and simulation (RQ3). In the following, we first describe the experimental setup used for our analysis, before describing each experiment in detail.

\subsection{Experimental Setup}
\label{sec:experimentalsetup}
We compared the predictive performance of our models on the two data sets to baseline models used in prior work \cite{cock2021early}.

\subsubsection{Data Sets}
\label{subsec:datasets}
The evaluation and validation data sets were collected in two different classroom experiments (see Table \ref{tab:demographics}).

\renewcommand{\arraystretch}{1.1}
\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lll@{}}
\toprule
& \textbf{Beer's Law Lab}  & \textbf{Capacitor Lab} \\                                    \midrule
\textbf{Number of students} & $254$ & $193$ \\
\midrule
\multirow{3}{*}{\textbf{Gender}} & Male: $53\%$ & \\ 
& Female: $43\%$ & N/A\\ 
& Other: $4\%$ &  \\                                                                        \midrule
\multirow{2}{*}{\textbf{Region}}  &A: $70\%$ & \multirow{2}{*}{USA}\\ 
& B: $30\%$ & \\                                                                            \midrule
\textbf{Education Level} & Vocational School & University \\                              \midrule
\multirow{2}{*}{\textbf{Field}} & Chemistry: $88\%$ & Physics majors: $17\%$\\
& Other: $12\%$ & Science/Engineering: $83\%$\\
\midrule
\textbf{Mean time in simulation} & 507s & 512s \\                                         \midrule
\textbf{Percentage label $1$}& $44\%$ & $51\%$\\
\bottomrule
\end{tabular}
}
\caption{Statistics of the data sets used for the experiments.}
\label{tab:demographics}
\end{table}
\renewcommand{\arraystretch}{1.0}

\textbf{Evaluation Data Set}. Using the Beer's Law Lab activity (see Section \ref{section:contextdata}), we collected data from $448$ laboratory technician apprentices of $10$ different vocational schools in a European country. The activity was performed directly in the classroom. We recorded students' interaction logs (clickstream data) as well as their responses to the ranking tasks. For our experiments, we removed participants who did not answer the ranking task ($23$ students), with an extremely short task duration (less than $2$ minutes), or with a low number of events (less than $10$ events). The final data set used for the experiment therefore consists of $254$ students. Prior to data collection, participants gave their informed consent to sharing the data for research, and all data was recorded in a completely anonymous way. Students could also participate in the learning activity without sharing their data for research. This study was approved by the responsible institutional review board (HREC number: 064-2021).

\textbf{Validation Data Set}. We used the data set collected by \cite{cock2021early} on the Capacitor Lab Activity (see Section \ref{section:contextdata}). It contains the interaction logs (clickstream data) and the ranking task responses of $193$ undergraduate Physics students of a US university. Students were all in their first year of studies and completed the activity as part of a mandatory homework assignment. Data was recorded in completely anonymous way and students had to give their informed consent prior to data collection. Moreover, students could participate in the learning activity without sharing their data for research. This study was approved by the responsible institutional review board (HREC number: 050-2020).

\subsubsection{Baseline Models}
\label{subsec:baseline}
We assessed the performance of our sequential models to more simple baseline models. Random forest (RF) models were successfully used in previous work \cite{cock2021early} to (early) predict students' level of conceptual understanding gained through interacting with an interactive simulation. \cite{cock2021early} experimented with neural network models and RF models with different type of features and did not find significant differences regarding predictive performance of the different model and feature combinations. We selected RF model with \textit{Action Span} features (\texttt{RF}) as a baseline for our experiments, as this encoding is most similar to our action-state sequences. The \textit{Action Span} features can be easily built from our state and action categories. For each time step $m$, the encoding of the triplet $(e'_m, s'_m, d_m)$ is similar to a one-hot encoded vector, where all entries are $0$ except the one representing $e'_m \times s'_m$ (state-action combination), which is equal to $d_m$. We therefore obtain a vector $v_m$ of dimensions $c_s \times c_e$. The raw interaction sequence $R_u$ for student $u\in\mathcal{U}$ then becomes $I_u = \{v_0, ..., v_{\tilde{n}_u\}}$. We flatten $I_u$ by summing all vectors $v_m$, resulting in a vector where each cell represents the amount of time in seconds the student spent doing each type of state-action combination. We then normalise the vector by the total duration of the interaction so that the model does not consider the length of each interaction, but rather the proportion of time spent on each condition.

\subsubsection{Optimisation Protocol}
Both \texttt{GRU} and \texttt{SA-GRU} are relatively sensitive to \textit{seeds} which have an influence on all weight initialisation. To temper the effects of randomness on the models' training, we used a cross validation with seed mitigation to optimise the neural network models. The usual nested cross-validation optimisation protocol was conducted for the baseline RF model. We evaluated performance of all models using the macro-averaged area under the ROC curve (AUC). 

\textbf{Optimisation for RF}. We optimised the \texttt{RF} model using a 10-fold nested cross validation stratified over the labels $L_u$. We use this step as an evaluation mean for the RF and as a basis for parameter optimisation for the GRU-based models. We ran the inner grid search on the following hyperparameters: the \textit{number of decision trees} $[3, 7, 9, 11, 13, 15, 17]$, the \textit{split criterion} $[gini, entropy]$, the \textit{maximum depth} $[5, 7, 9, 11, 13]$, the \textit{minimum samples split} $[3, 5, 7, 9, 11]$.
%\par We start by  conducting a 10-fold \textbf{nested} cross validation stratified across their conceptual understanding (what and how many concepts they grasped after interacting with the simulation) for the three algorithms. We optimise the random forest algorithm from scikit learn \cite{scikit-learn} on the \textit{number of decision trees} [3, 7, 9, 11, 13, 15, 17], the \textit{split criterion} [gini, entropy], the \textit{maximum depth} [5, 7, 9, 11, 13], the \textit{minimum samples split} [3, 5, 7, 9, 11]; the class weights [balanced subsample] and maximum features per base classifiers [automatic] are fixed parameters. 

\textbf{Optimisation for GRU and SA-GRU}. For the two sequential models, we performed initial protoyping using a 10-fold nested cross validation (using the same folds as for the RF model) and a small number of seeds. We trained both the \texttt{GRU} and \texttt{SA-GRU} for $150$ epochs, using a categorical crossentropy loss and an Adam optimiser. We tuned the following hyperparameters: dropout rate after the GRU layer $[0.02, 0.05]$ and the number of cells $[32, 64]$ in the GRU layers. The initial experiments demonstrated that: the selected hyperparameter values in the inner grid search were the same for a majority of the folds, the categorical cross entropy loss on the inner validation data set tended to converge after $20-30$ iterations, and predictive performance of the models seemed to vary depending on the seed. We therefore decided to choose a fixed architecture for the \texttt{GRU} and \texttt{SA-GRU} models and limit the number of epochs to $30$ for all our experiments. For Beer's Law Lab the selected parameters were a dropout rate of $0.02$ and $32$ units for the GRU layer. For the Capacitor Lab, we also use $32$ units in the GRU Layer and a dropout rate of $0.05$. We evaluated the models using 10-fold cross validation (based on the same outer folds as the RF model). To mitigate the potential effects of randomness, we trained both models over $n$ different seeds and averaged predictive performance across seeds. For our experiments on the full state-action sequences (see Sections \ref{sec:resrq1} and  \ref{sec:resrq3}), we used $n=60$ seeds. Since we observed only minor differences in predictive performance across seeds, we reduced the number of seeds to $n=10$ for our early prediction experiments (see Sections \ref{sec:resrq2} and  \ref{sec:resrq3}).

%We optimise the dropout rate for the SA-GRU [0.02, 0.05] as well as the number of GRU cells [32 or 64]. We train both GRU and SA-GRU on seed 193 with 150 epochs without early stopping, using a callback retrieving the model with the best validation score at the end of the 150 epochs. Once the optimal GRU/SA-GRU architecture has been selected, we re-run another gridsearch where the only hyperparameter we change is the seed [0, 16, 60,  3, 64, 69, 75, 96,  5, 77]. Finally, we run the optimal architecture on the optimal seed to compute the test scores for each fold.

%\textbf{Model Evaluation} \par We observe that the chosen sets of parameters in the architecture-gridsearch are often similar, and that the seed selection introduces minor variations across folds. To report fairer results and mitigate the potential effects of randomness, we re-train both models over 60 seeds on the most common selected architecture (from 1 to 60).  We decide to only run each algorithm for 30 epochs without early stopping nor callbacks to retrieve the model with the best validation score at the end. This design decision was based on the categorical cross-entropy loss and roc values measured on the validation sets during the \textit{nested cross validation} training phase: we observed on multiple instances (one of them shown in figure~\ref{fig:trainvalidation}) that the validation scores tended to plateau and not improve after 30 epochs approximately.

%\textbf{Early Predictions} 

\begin{comment}
\begin{figure}
\Description{}  % Alt text
\centering
\includegraphics[width=\columnwidth]{EDM-template/figures/design-decision.png}
\caption{Categorical cross-entropy loss and roc over 150 epochs for a SA-GRU algorithm initialised with seed 1.}
\label{fig:trainvalidation}
\end{figure}
\end{comment}

%%%%%%%%%% Research question 1: Full Sequence, ChemLab %%%%%%%%%%%%%%%%%%%%%
\subsection{RQ1: Full Sequence Prediction}
\label{sec:resrq1}
In a first experiment, we investigated whether our proposed models were able to predict students' level of conceptual understanding based on their interaction data. We used the evaluation data set collected with the Beer's Law Lab simulation to answer RQ1.

\textbf{Predictive Performance}. Figure \ref{fig:chemlabfullpred} illustrates the predictive performance in terms of AUC for the \texttt{GRU}, the \texttt{SA-GRU}, and the \texttt{RF} baseline. Both sequential models outperform the \texttt{RF} baseline: using \texttt{GRU} and \texttt{SA-GRU} models we improve the AUC by $~10\%$ ($AUC_{GRU} = 0.77$, $AUC_{SA-GRU} = 0.76$, $AUC_{RF} = 0.70$). We also observe that the \texttt{RF} model exhibits a higher variability across folds than the two sequential models. For those, the minimum AUC is close to $0.70$ ($AUC_{min,GRU} = 0.69$, $AUC_{min,SA-GRU} = 0.68$). In contrast, performance of the \texttt{RF} model drops below $0.6$ based on the fold ($AUC_{min,RF} = 0.58$). We also performed a preliminary analysis on model bias according to protected attributes. Specifically, we grouped the students based on the available protected attributes and computed predictive performance in terms of AUC separately for the different groups. We found that the \texttt{GRU} model is slightly biased towards male students ($AUC_{m,GRU}=0.78$, $AUC_{f,GRU}=0.73$), while the two other models do not show any gender bias. All models show a bias in terms of region, with a higher AUC for region A ($AUC_{A,GRU}=0.78$, $AUC_{A,SA-GRU}=0.78$,$AUC_{A,RF}=0.76$) than for region B ($AUC_{B,GRU}=0.69$, $AUC_{B,SA-GRU}=0.66$,$AUC_{B,RF}=0.63$).

\begin{figure}[!t]
\Description{AUC of the GRU for the Beer's Law Lab experiment: mean is 0.77, spread is around 0.12. AUC of the SA-GRU model: mean is 0.76, spread is around 0.15. AUC of random fores: mean is 0.7, spread is around 0.3.}
  \centering
  \includesvg[width=0.9\columnwidth]{figures/full-chemlab-bubbleplot.svg}
  \caption{AUC of the GRU, SA-GRU, and RF models on the evaluation data set collected from Beer's Law Lab. Predictions were made based on the complete sequential interaction data of the students.}
  \label{fig:chemlabfullpred}
\end{figure}

\textbf{Attention Interpretation}. While adding self-attention to the GRU does not increase predictive performance of the model (there is no significant difference in the performance of the \texttt{GRU} and \texttt{SA-GRU} model), the self-attention scores enable interpretation of the such black-box models. The heatmap in Fig. \ref{fig:attheatmapfullchemlab} shows the normalised attention scores for the \texttt{SA-GRU} model over $150$ time steps. For each student $u\in\mathcal{U}$, we extracted the output (dimension: $n_u \times f$) of the self-attention layer of the \texttt{SA-GRU} model (see Fig. \ref{fig:sagrudl}) and normalised it to make the attention scores comparable between models. We then averaged across all students. The number of students decreases rapidly with an increasing number of time steps (Fig. \ref{fig:chemlabfullpred} (top)). In fact, for $90\%$ of the students, $n_u \leq 150$.

We observe that the model seems to pay most attention to two of the states (\textit{green-red} and \textit{no absorbance}). The former state, \textit{green-red}, indicates a green laser colour and a red solution colour while the absorbance is measured. As expected, exploring with this parameter setting is important for solving the ranking task. The latter state, \textit{no absorbance}, indicates that the absorbance (outcome variable of the task) was not displayed, which makes solving the task impossible. Also the two other states (\textit{green-green} and \textit{absorbance}) seem to have phases of higher importance over time. For the \textit{no absorbance} state, we can see that the the model seems to pay less attention to it with an increasing number of time steps. Generally, the actual state of the simulation seems to be considered as more important than a specific action of the student. Regarding the action, the model seems to pay attention to state \textit{pdf}, which refers to students checking the task description and hence the configurations to be ranked. Also experimenting with \textit{concentration} and \textit{width} seems to have some importance. Interestingly, the importance of taking a \textit{break} varies over time steps. Finally, the model does not pay attention to the \textit{concentration-lab} action.

\begin{figure}[t]
\Description{histogram representing the number of students having at least x time steps. More people are included up until 10 time steps. There is a first dip at 30 time steps, where around 50 people stop interacting with the simulation. Less than 50 students have at least 150 time steps. Below is a graph showing the attention scores for the different features. The higher scores are for absorbance between 0 and 25 time steps and for the state green red between 10 and 25 time steps.}
  \centering
  \includegraphics[width=\columnwidth]{EDM-template/figures/attention-full-chemlab.png}
  \caption{Normalized attention scores for the SA-GRU over $150$ time steps (bottom). Number of students with $\mathbf{n_u \geq t}$ for $\mathbf{t = 1,...,150}$ (top).}
  \label{fig:attheatmapfullchemlab}
\end{figure}

\textit{In summary, this first experiment demonstrated that our proposed models yielded a $10\%$ increase in AUC over the RF approach suggested in previous work \cite{cock2021early}. Furthermore, the sequential models also exhibit a lower variance across folds. Finally, by adding self-attention to a GRU model, we were able to provide interpretations of what type of student exploration behavior will lead to successfully solving the task.}

%%%%%%%%%%%%%%%%% Research question 2: Early Prediction %%%%%%%%%%%%%%%%%%%%%
% write in paragraphs FP/TP, FN/TN on gender -> assessment on gender bias (with respect to protected attributes), region bias, year bias -> 
% => For LSTM, SSAN, RF (average roc per group over all seeds)
\subsection{RQ2: Early Prediction}
\label{sec:resrq2}
In our second experiments, we were interested in predicting students' level of understanding \textit{during} their interaction with the simulation. We therefore did not use all students' full interaction sequences, but used partial interactions up to a time step $l$ \jade{when the student went over that limit}. Therefore to build the features $F^{l,SA}_u$ for student $u\in\mathcal{U}$, we only used the interactions $I^l_u$ as a basis for building the features (see also Section \ref{sec:featextract}). We trained all our models for $l = 30, 40, 50, 60$. We did not make predictions earlier as we did not expect a model to be able to accurately predict conceptual understanding after only a few student actions. We further limited $l \leq 60$ as the number of students decreases for higher time steps (see also Fig. \ref{fig:attheatmapfullchemlab} (top) \jade{which indicates the amount of remaining students per time step}). At each time step $l$, we made predictions for students with state-actions sequences at each length $l$ (e.g. $\tilde{n}_u \geq l$). For students with shorter sequences (e.g., $\tilde{n}_u < l$), we used the last available prediction. We used the evaluation data set collected with Beer's Law Lab to answer RQ2.

\textbf{Predictive Performance}. Fig. \ref{fig:earlypredchemlab} illustrates the AUC of the different models for early prediction at $t = 30,40,50,60$. We again observe that the \texttt{RF} baseline model performs inferior to the sequential models. It achieves an AUC of $0.59$ after $30$ time steps and manages to only slightly improve over time with an AUC of $0.61$ after $60$ time steps. The AUC of the \texttt{RF} is $0.70$ for full sequence prediction (see Section \ref{sec:resrq1}), we therefore observe a strong increase in predictive performance when observing full sequences. It thus seems that the \texttt{RF} classifiers is not able to extract strong signal from early observations. The use of more elaborate sequential models leads to an up to $15\%$ increase in AUC ($AUC_{30,GRU} = 0.67$, $AUC_{30,SA-GRU} = 0.68$, $AUC_{60,GRU}$ $= 0.72$, $AUC_{60,SA-GRU} = 0.72$). Similar to the full sequences case, \texttt{RF} exhibits a much higher variance across folds than that our proposed models.

\begin{figure}[t]
  \centering
  \Description{Boxplot for the scores of the GRU, SA-GRU and RF at early time steps. The highest mean at time step=30 is for the SA-GRU, right below 0.7. For 40 timesteps, the highest mean is GRU, followed by SA-GRU, both around 0.65, while the mean of the RF is slightly below 0.6. For 50 time steps, SA-GRU performs slightly better than GU, both around 0.7, and the random dorest follows at around 0.65. In all cases, the spread of the boxplot is pretty wide, averaging towards 0.2. }
  \includesvg[width=\columnwidth]{figures/chemlab-early-boxplot.svg}
  \caption{Early predictive performance in terms of AUC for RF, GRU, and SA-GRU for the evaluation data set collected using Beer's Law Lab for $\mathbf{t = 30, 40,...,60}$.}
  \label{fig:earlypredchemlab}
\end{figure}

\textbf{Attention Interpretation}. Next, we investigated whether attention scores differed between an early prediction and a full sequence prediction model, i.e. whether the model paid attention to different features when making early predictions.

Figure \ref{fig:attheatmap30ChemLab} shows the normalised attention scores for the \texttt{SA-GRU} model trained to predict at time step $t=30$ The scores in the heatmap were calculated following the same procedure as for the full sequences case (see Section \ref{sec:resrq1}). Similar to our findings on full sequences, we observe that the states generally seem to be assigned higher scores than the actions. While we again observe that the \textit{no absorbance} and \textit{green-red} states have relatively higher scores, we also observe that these scores vary over time. The scores of the \textit{no absorbance} state clearly decrease over time. This finding might suggest that many students realise during their first $10-15$ interactions with the simulation that the absorbance display should be turned on (by default, transmittance is displayed). In contrast, the scores of the \textit{green-red} state increase over time, indicating that after being able to observe the outcome variable (absorbance), it is important to select the optimal colours for laser (green) and solution (red). For the actions, we observe the same picture as for the full predictions. The \textit{concentration-lab} action gets little attention (it is probably also a rare action), while manipulating \textit{width} and \textit{concentration} gets similar attention over time. Checking the task description is mainly important early on. The model does not pay attention to \textit{break} for the first $10$ time steps. We hypothesise that `thinking' breaks do not occur often during initial interaction when students are still focused on understanding the task and have not yet started their exploration.\\

\begin{figure}[t]
\Description{Attention scores for the SA-GRU which was trained for interactions up until 30 time steps. Most attention is given to the state no absorbance, especially until the 12th time step, where it is above 0.02. Then, it is also given to the green red state from the 12th time step on at a lesser scale (higher than 0.01). }
  \centering
  % [trim=left bottom right top, clip]
  \includegraphics[trim = 0cm 0.7cm 8.5cm 0cm, clip,width=\columnwidth]{EDM-template/figures/attention-early30-chemlab.pdf}
  \caption{Normalised attention scores for SA-GRU trained for predicting at $\mathbf{t = 30}$ time steps for Beer's Law Lab.}
  \label{fig:attheatmap30ChemLab}
\end{figure}

\textit{In summary, our second set of experiments showed that in case of early prediction, the use of a GRU or SA-GRU model leads to even larger performance increases than in case of full sequences. Depending on the time step, we observe improvements in AUC of $15\%$ compared to the RF baseline. Furthermore, the RF again shows high variability with drops in AUC down to $0.50$. We are again able to provide meaningful interpretations of the attention weights, which is a promising basis for targeted intervention.}


% \subsection{RQ3: Transferring to a Different Setting}
\subsection{\jade{RQ3: Generalisation}}
\label{sec:resrq3}
In our last experiment, we were interested in assessing the generalisability of the developed models. While both learning activities were based on a ranking task, the underlying simulation as well as the population are different. We therefore evaluated our models on the transfer data set collected from the Capacitor Lab simulation.

\textbf{Prediction on Full Sequences}. We first evaluated the generalisability of the different model by predicting on the full interaction sequences of the validation data set. Figure \ref{fig:fullpredcap} illustrates the predictive performance in terms of AUC for the \texttt{GRU}, the \texttt{SA-GRU}, and the \texttt{RF} baseline. We observe that all the models achieve a very high AUC for the Capacitor Lab data set. The sequential models achieve an AUC of $0.96$ (\texttt{GRU}) and $0.96$ (\texttt{SA-GRU}) respectively, while the AUC of the \texttt{RF} baseline is $0.95$. Again the \texttt{RF} baseline model shows higher variability, achieving a minimum AUC of $0.86$. For the \texttt{GRU} and \texttt{SA-GRU}
models, we achieved a minimum AUC of $0.9$ and $0.89$ respectively. For Capacitor Lab, we ran the same bias analysis on protected attributes as for Beer's Law Lab, showing that models are not biased with respect to field (the only known protected attribute for this data set).
 
While the \texttt{SA-GRU} model does not outperform the other two models, we again extracted the attention weights of this model and interpreted them. Figure \ref{fig:attheatmapfullcapacitor} shows the normalised attention scores of the \texttt{SA-GRU} models over a $100$ time steps. We chose to limit to $100$ time steps as for $90\%$ of the students $\tilde{n}_u \leq 100$. Again, the scores displayed in the heatmap were calculated using the procedure described in Section \ref{sec:resrq1}. Similar to our findings on Beer's Law Lab, we observe that the states (\textit{stored energy}, \textit{closed circuit}) receive higher attention than the actions. For \textit{stored energy}, attention scores increase up to time step $30$ and then decrease again after time step $60$. We assume that students needed some time to explore the simulation and figure out that the stored energy display needs to be turned on (it is by default turned off in the simulation). For the \textit{closed circuit} state, attention scores decrease over time, but there are always phases of increased activity. In order to be able to solve the ranking task, it is important to experiment with the closed as well as the open circuit, as detected by the model. The model also seems to pay attention to actions related to \textit{voltage}, \textit{plate area}, and \textit{plate separation}, which are the other three components in the simulation that influence the stored energy. Moreover, \textit{breaks} are important for different phases within the sequences. Hence, the model seems to detect when students take a thinking break and considers that as important.

\begin{figure}[!t]
\Description{Capacitor Scores for the GRU, SA-GRU and RF. All models have a mean of around 0.95, with the mean+std equal to 1. }
  \centering
  \includesvg[width=\columnwidth]{figures/full-capacitor-bubbleplot.svg}
  \caption{AUC of the GRU, SA-GRU, and RF models on the validation data set collected from CapacitorLab. Predictions were made based on the full interaction data of the students.}
  \label{fig:fullpredcap}
\end{figure}

\begin{figure}[!t]
\Description{On top is a histogram showing the distribution of the students throughout different time steps. Most people (193) are kept until 20 time steps. At 60 time steps, less than 100 students are still present in the corpus. Most attention is given to the circuit state (0 if closed, 1 if opened): the scores are higher than 0.014 until around 20 time steps, and it is still higher than the other action features than the action features. The second highest attention score is for the stored energy. It goes above 0.008 from 15 time steps on.}
  \centering
  \includegraphics[width=\columnwidth]{EDM-template/figures/attention-full-capacitor.png}
  \caption{Normalized attention scores for CapacitorLab for the SA-GRU over $150$ time steps (bottom). Number of students with $\mathbf{n_u \geq t}$ for $\mathbf{t = 1,...,150}$ (top).}
  \label{fig:attheatmapfullcapacitor}
\end{figure}

\textbf{Early Prediction}. Next, we also trained the different models for early prediction on Capacitor Lab. Figure \ref{fig:earlypredcaplab} shows the AUC of the evaluated models for prediction on $t=30,40,50,60$ time steps. We see that the AUC of the two sequential model is close to $0.80$ already after observing $30$ student interactions ($AUC_{30,GRU} = 0.8$, $AUC_{30,SA-GRU} = 0.81$). Predictive performance of the \texttt{RF} model is slightly lower ($AUC_{30,RF} = 0.76$). After $60$ time steps, all the models achieve an AUC larger than $0.8$ ($AUC_{60,GRU} = 0.9$, $AUC_{60,SA-GRU} = 0.9$, $AUC_{60,RF} = 0.88$). We observe that all three models show a similar variability under this task.

\begin{figure}[!t]
\Description{AUC scores of the capacitor lab for different time steps. The means increase from 0.8 to 0.92 as the time steps increase. All performances are comparable, with the random forest scoring slightly below GRU and SA-GRU. }
  \centering
  \includesvg[width=\columnwidth]{figures/capacitor-early-boxplot.svg}
  \caption{AUC of the GRU, SA-GRU, and RF models for early prediction ($\mathbf{t = 30, 40, ..., 60}$) on Capacitor Lab.}
  \label{fig:earlypredcaplab}
\end{figure}

\textit{In summary, our results demonstrate that the proposed models can be transferred to a different learning environment and population. In case of full interaction data, the performance of the models is inline with the RF baseline, in case of early prediction, the sequential models outperform the baseline. Furthermore, the addition of self-attention again enabled us to identify the key points in the exploration process.}

==> context.tex <==
\section{Learning Environments}\label{section:contextdata}
%\section{Learning environments}
% Describe chemlab + capacitor (shorter)
% Does the paper provide detail on the demographics of the population involved in the study?
% Does the paper describe how participants’ privacy rights were respected in the data collection process?
The PhET interactive simulations\footnote{https://phet.colorado.edu/} allow students to explore natural phenomena using different parameter configurations and ideally infer the underlying principles on their own. A large body of research has focused on analysing students' inquiry strategies using these simulations, usually coupled with an explicit task to be solved using the simulation \cite{yehya2019learning}. To evaluate the (early) prediction models presented in this paper, we used a ranking task which we adapted to two different simulation environments. \jade{For each ranking task, the values of the variables presented in the task are outside the range provided by the simulation. Hence, students need to inquire the system to uncover the appropriate equations and plug in the numbers as answers in the ranking task.}
% To be able to solve the ranking task, students need to infer the principles governing the simulation.
%The methods presented in this paper were evaluated with two data sets collected from classroom experiments in which students solved inquiry-based learning tasks using two of the PhET interactive simulations\footnote{https://phet.colorado.edu/}. While different simulations were used for each data set, the associated learning tasks were designed in a similar way thus enabling the application of the same analysis methods for both data sets.

\begin{figure} 
\Description{The two learning environments used to collect both datasets in this paper are depicted: the capacitor lab on the left, and the beer's law lab on the right.} 
\centering \includegraphics[width=\columnwidth]{EDM-template/figures/Fig_phet_envs.JPG} \caption{The two learning environments used in this study, the Capacitor Lab (A) and the Beer's Law Lab (B).} 
\label{fig:phet-envs} 
\end{figure}

\begin{figure}[!t]
\Description{TODO}  % Alt text
\centering
\subfloat[Task for the Capacitor Lab simulation \cite{cock2021early}. ]{\includegraphics[width=\columnwidth]{EDM-template/figures/caplab_task.png}}\\
\subfloat[Task for the Beer's Law Lab simulation. ]{\includegraphics[width=\columnwidth]{EDM-template/figures/fig_ranking_beer.pdf}}\label{fig:ranktaskchemlab}
\caption{Ranking tasks for the two interactive simulations.}
\label{fig:ranktask}
\end{figure}

\textbf{Capacitor Lab}. The PhET Capacitor Lab simulation\footnote{https://phet.colorado.edu/en/simulations/capacitor-lab} provides students with the possibility to manipulate different parameters of an electric circuit (plate area, plate separation, applied voltage, open/close the circuit), to help them understand how each parameter influences the capacitance of a plate capacitor as well as the energy stored in that capacitor (see Fig. \ref{fig:phet-envs}A). Previous work \cite{cock2021early} designed an inquiry-based learning activity for this simulation using a ranking task. Specifically, students were asked to rank four different configurations according to the stored energy saved in the plate capacitor (see Fig. \ref{fig:ranktask}a). The four configurations were created by first loading the plate capacitor using two parameter configurations in a closed circuit (A and B), followed by opening the switch to disconnect the capacitor from the circuit and changing the parameters to obtain the final configurations to be ranked (1, 2, 3, and 4). The authors also suggested a tree-based approach to label the $24$ possible solutions based on conceptual understanding. For this paper, we will use the binary labels suggested by \cite{cock2021early} to divide students into a group with an \texttt{advanced understanding} of stored energy (i.e., for both open and closed circuits) and a second group with a conceptual understanding limited to the closed circuit, denoted as \texttt{limited understanding}.

\textbf{Beer's Law Lab}. The PhET Beer's Law Lab simulation\footnote{https://phet.colorado.edu/en/simulations/beers-law-lab} allows students to explore how light is absorbed in a solution and which factors influence the measured absorbance (Fig. \ref{fig:phet-envs}B). In this environment, the students can manipulate the following components: the wavelength $\lambda$ of the light beam, the width of the container (representing the light's path length $L$ through the solution), the substance of the solution (changing its colour), and its concentration $c$. By experimenting with these components, in the ideal case, students can infer Beer's Law, which describes how each parameter influences the measured absorbance: $ A = \epsilon_\lambda * L * c $. Based on the inquiry-based learning task presented by \cite{cock2021early}, we developed a ranking task that can be solved with Beer's Law Lab. Students were presented with four flasks that varied in width as well as in the color and concentration of the solution they contained (Fig. \ref{fig:ranktask}b). Given a light beam of a specific wavelength, students were asked to rank the four flasks by the measured absorbance. It is important to note that the values chosen for the four flasks were not available in the simulation in order to prevent students from obtaining the correct ranking by simply replicating the flasks. To label the submitted rankings, we used the tree-based approach introduced in previous work \cite{cock2021early}. We classified each of the $24$ possible rankings according to the level of conceptual understanding (Fig. \ref{fig:labelschemlab}). Specifically, for each ranking, it was determined whether the influence of i) the substance's concentration, ii) the container's width and iii) the colour difference between light beam and solution was understood or not. Rankings were then grouped by the number of concepts understood that they represented. Rankings representing $0$ or $1$ concepts understood were then labelled as \texttt{limited understanding}, while rankings representing $2$ or $3$ concepts were labelled as \texttt{advanced understanding}.

\begin{figure}[t]
\Description{TODO}  % Alt text
\centering
\includegraphics[width=\columnwidth]{EDM-template/figures/fig_labels_beer.pdf}
\caption{The tree used to map the rankings to different levels of conceptual understanding. The numbers in parentheses indicate the number of submissions for the ranking.}
\label{fig:labelschemlab}
\end{figure}

%\begin{figure}
%\Description{Four flasks: 1) green solution, width of 3 cm, concentraion of $5microMol/L$, 2) green solution, width of 3cm, concentraion of 200micro mol per liter, 3) red solution, width of 4.5 cm, concentration of 150 micro mol per liter. 4) red solution, width of 0.75cm, concentration of 250 micro mol per liter.}  % Alt text
%\centering
%\includegraphics[width=\columnwidth]{EDM-template/figures/fig_ranking_labels.pdf}
%\caption{A) The ranking task presented for the Beer's Law Lab. B) The tree used to map the rankings to different levels of conceptual understanding. The numbers in parentheses indicate the number of submissions for the ranking. }
%\label{fig:ranking-task-chemlab}
%\end{figure}


%All experiments described in this paper are conducted with interaction logs generated by the PhET interface. Those were collected during user studies in which we evaluated students' inquiry and problem solving skills. In the rest of this section, we describe the learning activities, pre-processing of the interaction logs, features extractions and model architectures implemented to classify students according to their conceptual understanding of different scientific topics.

%\textbf{Capacitor Lab Activity.} To assess the generalizability of the presented methods, a second data set was used in the analyses. This data was collected in a previous work \cite{cock2021early} involving experiments with the Capacitor Lab simulation. This environment provides students with the possibility to manipulate different parameters of an electric circuit (plate area, plate separation, applied voltage, open/close the circuit) to help them understand how each of them influences the energy stored by a plate capacitor (Fig. \ref{fig:phet-envs}B). Analogously to the Beer's Law Lab activity, a ranking task was designed and presented to the students. In this case, students had to rank four different configurations of plate capacitors by the energy they stored. Using the same tree-based approach, the submitted rankings were then labeled and classified into two main groups: the first group included all the rankings representing a complete understanding (i.e., both open and closed circuits), whereas rankings in the second group represented an understanding limited to the closed circuit. For more details on the design of the ranking task as well as the labeling procedure, please refer to the original work \cite{cock2021early}.

==> method.tex <==
\section{Method}
\label{sec:method}
We are interested in creating \textit{generalisable models} to (early) predict the level of conceptual understanding students will achieve after interacting with a simulation. Formally, our goal is to predict, for each student, a binary label representing their level of conceptual understanding. To address this binary classification task, we propose a pipeline consisting of the four steps illustrated in Fig. \ref{fig:datapipeline}. We first pre-process the data into event logs and extract so-called state-action sequences from these event logs. We then build different types of deep neural network models to perform the classification task. In what follows, we first formalise the addressed problem, before describing each step of the pipeline in detail.

\begin{figure*}[t]
\Description{The data pipeline consist in 1) the data processing (states and actions are combined, and the shortest 60\% breaks are discarded as being non relevant to the user interaction), 2) The feature extraction part (states and actions are categorised into a small number of groups), 3) model building (the data is fed into a GRU and an attention GRU to (early) predict students' conceptual understanding).}  % Alt text
\centering
\includegraphics[trim= 0.0 0.0 0cm 4.5cm,width=0.8\textwidth]{EDM-template/figures/methodspipeline.pdf}
\caption{Our model building pipeline consists of three steps: we first extract the logs into sequences of events and states. We then categorise the states and events to build state-action sequences. Finally we feed the features into variations of GRU models.}
\label{fig:datapipeline}
\end{figure*}

\begin{figure*}[!t]
\Description{Architecture of our GRU model with one unrolled GRU layer: the input time steps are fed sequentially into the recurrent cells of the GRU layer. The output of the last GRU cell is fed to the dense layer which is then SoftMax activated to determine the probability of the student belonging to each of the 2 classes.}  % Alt text
\centering
\includegraphics[trim= 0.0 0.0 0cm 4.5cm, clip,width=0.7\textwidth]{EDM-template/figures/GRUDL.pdf}
%   \includesvg[width=\columnwidth]{figures/GRUDL.svg}
\caption{Architecture of our \texttt{GRU} model with one unrolled GRU layer: the input features are fed sequentially into the recurrent cells of the GRU layer. The output shape of each layer is given: $|U|$ denotes the number of users, $\tilde{n} = \max_{u\in\mathcal{U}} \tilde{n}_u$, $cell$ the number of GRU cells, and $f$ the number of features in the input matrix.}
\label{fig:grudl}
\end{figure*}


\subsection{Problem Formalisation}
We consider $\mathcal{U}$ to be the set of students participating in the learning activity. During this learning activity, students use an interactive simulation in order to rank four different configurations according to a specific criterion (see Section \ref{section:contextdata} for details on the ranking tasks). We denote the set of possible answers to the ranking task as $\mathcal{A}$ and the answer of a student $u \in \mathcal{U}$ to this ranking task $a_u \in \mathcal{A}$. Based on their answers, we assign a label $L_u \in \{0, 1\}$ to each student $u \in \mathcal{U}$. This mapping $m$ is a direct function of students' answers and can be formalised as  $m: a_u\in \mathcal{A} \longmapsto L_u \in \{0, 1\}$ for $u\in \mathcal{U}$. For both lab activities, label $1$ denotes \texttt{advanced understanding} and label $0$ \texttt{limited understanding}.

\par To solve the ranking task, students interact with the simulation and investigate the factors influencing the dependent variable (absorbance in case of Beer's Law Lab, stored energy in case of Capacitor Lab). Their full and non-processed sequence of events in the simulation is denoted as:
\vspace{-5mm}

\begin{equation}\label{eq:rawsequence}
    R_u = \{(e_0, s_0, d_0), ..., (e_{n_u-1}, s_{n_u-1}, d_{n_u-1})\}
\vspace{-2mm}
\end{equation}

where $e_m$ is the $m^{th}$ \textit{event} $e$ , $s_m$ is the \textit{state of the simulation} at time step $m$, and $d_m$ denotes the \textit{duration of event} $e_m$ in \textit{state} $s_m$.
We denote the partial sequence of student $u \in\mathcal{U}$ from the first to the $l^{th}$ event as $R_u^l=\{(e_0, s_0, d_0), ..., (e_{l-1}, s_{l-1}, d_{l-1})\}$ with the value $l\in[1, n_u)$.
To clarify the notion of \textit{duration} and \textit{time steps}, we introduce $\|R_u\|_{duration} = t_u$ where $t_u$ denotes the total time in seconds spent by student $u$ on the simulation. We then denote $\|R_u\|_{timestep} = n_u$ where $n_u$ denotes the total number of events performed by student $u$ in sequence $R_u$.

Hence, training an (early) students' conceptual understanding predictor $\mathcal{E}$ with interactions $R_u$ and conceptual label $L_u$ after a number of interactions $\bf{n}_u$ becomes an optimisation problem, aimed to find model parameters $\theta$ that maximise the expectation on the following objective function (i.e., predict the correct label, given interactions) over a dataset $\mathbb G$:
\vspace{-10mm}

\begin{equation}
\tilde{\theta} = \underset{\theta}{\operatorname{argmax}} \mathop{\mathbb{E}}_{(R_u, L_u)\in \mathbb{G}}  L_u = \mathcal{E}(R_u^{\bf{n}_u} \;|\; \theta)
\label{eq:problem-definition}
\vspace{-2mm}
\end{equation}

In what follows, we describe the steps carried out to solve this problem from pre-processing until model building.  

\subsection{Data Pre-Processing}
From the log data, we extract the sequence of events of a student $u$ as follows: anything between a mouse click and a mouse release qualifies as an \textit{action}. Each \textit{action} can be described by its \textit{duration} and the \textit{component} the action is performed on, and is conducted in a specific \textit{simulation state}. Anything between a mouse release and a mouse click qualifies as a \textit{break}. Similarly, \textit{breaks} are conducted in a specific \textit{state} and have a specific \textit{duration}.
All \textit{actions} and \textit{breaks} generated by a student $u\in\mathcal{U}$ are sorted chronologically to form the raw interaction sequence of a user $u\in\mathcal{U}$, $R_u$ as per Eq. \ref{eq:rawsequence}, where events can be both \textit{actions} or \textit{breaks}.

Some \textit{breaks} in student interactions can be indicative of reflective, observational or distracted periods. Other \textit{breaks} can occur naturally throughout a student's interaction when the mouse moves from one element to the other \cite{wang2021examining}. The latter might introduce undesired noise and hinder student classification over their conceptual understanding, not unlike stop words negatively influence sentiment analysis tasks in the domain of natural language processing, as an example \cite{ghag2015comparative}. To maximise the retention of informative periods of inactivity, we therefore discard for each student $u\in\mathcal{U}$ their $60\%$ of shortest breaks. We are left with $R_u = \{(e_0, s_0, d_0), ..., (e_{\Tilde{n}_u-1}, s_{\Tilde{n}_u-1}, d_{\Tilde{n}_u-1})\}$ with $\Tilde{n}_u \leq n_u$, the final sequence of triplets of events $e_m$ occurring in state $s_m$ and of duration $d_m$ for student $u\in\mathcal{U}$ at time $m\in[0, t_u)$. \jade{The new sequence contains $\tilde{n}_u$} event triplets, i.e., \textit{timesteps}.

\begin{figure*}[!t]
\Description{\texttt{SA-GRU} architecture with the depiction of the attention mechanism for timestep $t$.}  % Alt text
\centering
\includegraphics[width=0.86\textwidth]{EDM-template/figures/SAGRU.pdf}
%   \includesvg[width=\columnwidth]{figures/SAGRUDL.svg}
\caption{\texttt{SA-GRU}'s architecture with the attention mechanism. The output shape of each layer is given: $|U|$ denotes the number of students, $\tilde{n} = \max_{u\in\mathcal{U}} \tilde{n}_u$, $f$ is the number of dimension in the state-action features, and $cells$ is the number of GRU cells.}
\label{fig:sagrudl}
\end{figure*}

\subsection{Feature Extraction}
\label{sec:featextract}
% Be more general -> state of the siulation + for chemlab it would look like that, and for capacitor lab it would look like that
\jade{The data logging of the PhET environments captures any click targeting an "interactive" component as well as the state of the simulation in case one of these "clicks" changes the value of a variable/multiple variables in the system. This fine-grained logging results in high dimensional simulation states $s$ and a high number of different events $e$. Before creating feature vectors for each time step $m$, we therefore categorise the obtained events and states into meaningful components. We divide all possible \textit{simulation states} into two groups: a) helpful or b) unhelpful to solve the problem. We then ponder whether some of the \textit{helpful states} can be grouped such that the level of information received by the student is the same independent of the state within the group. We proceed in a similar way for the events. While this categorisation procedure is generalisable over different platforms, whether a simulation state or event is helpful depends on the actual task.}

\jade{\textbf{State-Action Categorisation for Capacitor Lab}. For the Capacitor Lab activity, we use the state and action categorisation defined in \cite{cock2021early}. By applying the above pipeline, we qualify each state $s_m \in (e_m, s_m, d_m)$ into one of the following groups: 1) closed circuit - stored energy displayed, 2) open circuit - stored energy displayed, 3) closed circuit - stored energy not displayed, and 4) open circuit - stored energy not displayed. Since stored energy is the dependent variable in the ranking task, displaying the stored energy is essential for solving the task. The relationship between the parameters (plate area, plate separation, battery voltage) and stored energy differs for closed and open circuits. Moreover, we map each event $e_m \in (e_m, s_m, d_m)$ into one of the following actions: 1) manipulating battery voltage, 2) manipulating plate area, 3) manipulating plate separation, 4) break, 5) other (any other action). }

% \textbf{State-Action Categorisation for Capacitor Lab}. For the Capacitor Lab activity, we use the state and action categorisation defined in \cite{cock2021early}. Consequently, we categorise each state $s_m \in (e_m, s_m, d_m)$ into one of the following four groups: 1) closed circuit - stored energy displayed, 2) open circuit - stored energy displayed, 3) closed circuit - stored energy not displayed, and 4) open circuit - stored energy not displayed. Since stored energy is the dependent variable in the ranking task, displaying the stored energy is essential for solving the task. The relationship between the different parameters (plate area, plate separation, battery voltage) and stored energy differs for closed and open circuits. Moreover, we map each event $e_m \in (e_m, s_m, d_m)$ into one of the following actions: 1) manipulating battery voltage, 2) manipulating plate area, 3) manipulating plate separation, 4) break, 5) other (any other action). 

\vspace{-1mm}
\jade{\textbf{State-Action Categorisation for Beer's Law Lab}. There are four independent variables that influence the dependent variable \textit{absorbance} of the ranking task: the \textit{laser colour}, the \textit{solution colour}, the \textit{concentration} of the solution, and finally the \textit{width} of the container. Consequently, we categorise each state $s_m \in (e_m, s_m, d_m)$ into one of those 4 groups: 1) green-green (absorbance: displayed, laser colour: green, solution colour: green), 2) green-red (absorbance: displayed, laser colour: green, solution colour: red), 3) absorbance displayed (absorbance: displayed, laser colour: not green and/or solution colour: neither red nor green), 4) not observed (absorbance: not displayed). To solve the ranking task depicted in Fig. \ref{fig:ranktaskchemlab}, students need to understand how the \textit{width} and \textit{concentration} interact with the \textit{absorbance} when the \textit{solution colour} is either red or green and when the \textit{laser colour} is green, i.e., states 1) and 2). The \textit{width} and the \textit{concentration} share a linear dependency with the \textit{absorbance} and are both colour agnostic. As long as the absorbance is observed, those relations can be discovered no matter the colour of the laser or the solution, i.e., state 3. Furthermore, we process each event $e_m \in (e_m, s_m, d_m)$ into one of those categories: 1) width (width slider is moved), 2) concentration (concentration slider is moved), 3) pdf (students are reading the instructions from the ranking task), 4) concentration lab (students are interacting with the second simulation available directly from the Beer's law lab), 5) breaks, 6) other.}

% \textbf{State-Action Categorisation for Beer's Law Lab}. There are four independent variables that influence the dependent variable \textit{absorbance} of the ranking task: the \textit{laser colour}, the \textit{solution colour}, the \textit{concentration} of the solution, and finally the \textit{width} of the container. Consequently, we categorise each state $s_m \in (e_m, s_m, d_m)$ into one of those 4 groups: 1) green-green (absorbance: displayed, laser colour: green, solution colour: green), 2) green-red (absorbance: displayed, laser colour: green, solution colour: red), 3) absorbance displayed (absorbance: displayed, laser colour: not green and/or solution colour: neither red nor green), 4) not observed (absorbance: not displayed). To solve the ranking task depicted in Fig. \ref{fig:ranktaskchemlab}, students need to understand how the \textit{width} and \textit{concentration} interact with the \textit{absorbance} when the \textit{solution colour} is either red or green and when the \textit{laser colour} is green, i.e., states 1) and 2). The \textit{width} and the \textit{concentration} share a linear dependency with the \textit{absorbance} and are both colour agnostic. Consequently, as long as the absorbance is observed, those relations can be discovered no matter the colour of the laser or the solution, i.e., state 3. Furthermore, we process each event $e_m \in (e_m, s_m, d_m)$ into one of those categories: 1) width (width slider is moved), 2) concentration (concentration slider is moved), 3) pdf (students are reading the instructions from the ranking task), 4) concentration lab (students are interacting with the second simulation available directly from the Beer's law lab), 5) breaks, 6) other (any other actions including those related to the laser's colour and the solution's colour as both are implicitly included in the state encoding).

\textbf{State-Action Sequences}. After the categorisation step, each $e_m \in (e_m, s_m, d_m)$ will have been replaced by $e_m'$, its corresponding event category, and each $s_m \in (e_m, s_m, d_m)$ will have been replaced by $s_m'$, its corresponding state mapping. For each timestep $m$, we encode $s'_m$ as a one-hot-encoded vector $v^{s'}_m$ of $c_s$ cells (with $c_s$ denoting the number of different state categories for the simulation), where all entries are $0$ except the one corresponding to $s'_m$, which is equal to $1$. We also transform $e'_m\in(e'_m, s'_m, d_m)$ into a one-hot-encoded vector $v^{e'}_m$ of $c_e$ cells (with $c_e$ denoting the number of different event categories for the simulation), where all entries are $0$ except the one corresponding to $e'_m$, which is equal to $d_m$. Finally, for each time step $m$, we replace each triplet $(e'_m, s'_m, d_m)$ by the concatenation of both vectors $v^{s'}_m$ and $v^{e'}_m$. 
For each student $u\in\mathcal{U}$, the interaction sequence $R_u$ can now be formulated as $\{[v^{s'}_0, v^{e'}_0], ..., [v^{s'}_{t_u-1}, v^{e'}_{t_u-1}]\}$.
We then normalise the sequences on the $v^{e'}_0$ dimension resulting in the final action sequence $F^{SA}_u$ for student $u\in\mathcal{U}$.

\vspace{0mm}
\subsection{Model Building}
In this paper, we are interested in creating a conceptual understanding prediction model that can accurately predict the conceptual understanding label $L_u$ for student $u$, given the extracted features $F_u^{SA}$. To this end, we rely on two types of models, both based on a \textit{Gated Recurrent Unit} (GRU) network \cite{cho2014properties}. GRUs are a type of Recurrent Neural Networks (RNNs), whose specificity is to allow the transmission of information over time. To process sequential data, RNNs are composed of $r$ recurrent cells arranged successively such that the output of one becomes the input of the next one, as illustrated on Figure~\ref{fig:grudl}. Their relative simplicity enables GRUs to handle smaller datasets (as those in our hands) than the more complex long short-term memory cells (LSTM), which contain an additional output gate~\cite{lstmchung2014empirical, lstmgruber2020gru}.

The first type of model is based on a GRU combined with a Dense layer (\texttt{GRU}), as shown in Figure \ref{fig:grudl}. Specifically, the extracted features $F^{SA}$ are fed into a neural architecture composed of a \emph{GRU}, a \emph{dropout} layer and a \emph{Dense} layer (with Softmax activation) having a hidden size of $1$. The model outputs the probability the student $u$ will gain advanced (label $1$) or limited (label $0$) understanding.

The second type of model is based on a Self-Attention-based Gated-Recurrent-Unit (\texttt{SA-GRU}), as shown in Figure \ref{fig:sagrudl}. In 2014, the concept of an \textit{Additive Attention} layer, also called \textit{Bahdanau attention} was introduced to improve statistical machine translation \cite{bahdanau2014neural}. Rather than using it to understand the context of words across languages, we use it to identify the pivotal moments in students' interactions with the simulation. We first take the raw extracted features $F^{SA}$ as the \textit{query}, \textit{key} and \textit{value} input matrices to our self-attention mechanism implemented as in \cite{attentionimplementation}. We then concatenate the attention output with the input features along each time step and feed this matrix to a GRU layer. Its latest output will directly be given to the dropout layer before passing through the final Dense layer which uses a Softmax activation (analogously to the \texttt{GRU} model). Though more complex than \texttt{GRU} and consequently more subject to overfitting on smaller datasets, \texttt{SA-GRU}'s attention weights can be used to understand what dimension of our features are important for the final prediction, and when that importance is emphasised over time. These aspects are fundamental to enable interpretability on such complex yet effective models. 


==> results.tex <==
\section{Experimental Evaluation}
\label{sec:results}
We evaluated our (early) prediction models on two data sets collected using the ranking task activities on the PhET Beer's Law Lab and Capacitor Lab simulations (see Section \ref{section:contextdata}). We used the data set that we collected using the Beer's Law Lab activity as an \textit{evaluation data set} to assess to what degree student interaction data within the simulation is predictive for their obtained conceptual understanding (RQ1) and whether our models are able to predict students' conceptual understanding at the end of the task \textit{early} on (RQ2). We then used the data that was collected by previous work \cite{cock2021early} using the Capacitor Lab activity as a \textit{validation data set} to assess the transferability of our proposed models to a different population and simulation (RQ3). In the following, we first describe the experimental setup used for our analysis, before describing each experiment in detail.

\subsection{Experimental Setup}
\label{sec:experimentalsetup}
We compared the predictive performance of our models on the two data sets to baseline models used in prior work \cite{cock2021early}.

\subsubsection{Data Sets}
\label{subsec:datasets}
The evaluation and validation data sets were collected in two different classroom experiments (see Table \ref{tab:demographics}).

\renewcommand{\arraystretch}{1.1}
\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lll@{}}
\toprule
& \textbf{Beer's Law Lab}  & \textbf{Capacitor Lab} \\                                    \midrule
\textbf{Number of students} & $254$ & $193$ \\
\midrule
\multirow{3}{*}{\textbf{Gender}} & Male: $53\%$ & \\ 
& Female: $43\%$ & N/A\\ 
& Other: $4\%$ &  \\                                                                        \midrule
\multirow{2}{*}{\textbf{Region}}  &A: $70\%$ & \multirow{2}{*}{USA}\\ 
& B: $30\%$ & \\                                                                            \midrule
\textbf{Education Level} & Vocational School & University \\                              \midrule
\multirow{2}{*}{\textbf{Field}} & Chemistry: $88\%$ & Physics majors: $17\%$\\
& Other: $12\%$ & Science/Engineering: $83\%$\\
\midrule
\textbf{Mean time in simulation} & 507s & 512s \\                                         \midrule
\textbf{Percentage label $1$}& $44\%$ & $51\%$\\
\bottomrule
\end{tabular}
}
\caption{Statistics of the data sets used for the experiments.}
\label{tab:demographics}
\end{table}
\renewcommand{\arraystretch}{1.0}

\textbf{Evaluation Data Set}. Using the Beer's Law Lab activity (see Section \ref{section:contextdata}), we collected data from $448$ laboratory technician apprentices of $10$ different vocational schools in a European country. The activity was performed directly in the classroom. We recorded students' interaction logs (clickstream data) as well as their responses to the ranking tasks. For our experiments, we removed participants who did not answer the ranking task ($23$ students), with an extremely short task duration (less than $2$ minutes), or with a low number of events (less than $10$ events). The final data set used for the experiment therefore consists of $254$ students. Prior to data collection, participants gave their informed consent to sharing the data for research, and all data was recorded in a completely anonymous way. Students could also participate in the learning activity without sharing their data for research. This study was approved by the responsible institutional review board (HREC number: 064-2021).

\textbf{Validation Data Set}. We used the data set collected by \cite{cock2021early} on the Capacitor Lab Activity (see Section \ref{section:contextdata}). It contains the interaction logs (clickstream data) and the ranking task responses of $193$ undergraduate Physics students of a US university. Students were all in their first year of studies and completed the activity as part of a mandatory homework assignment. Data was recorded in completely anonymous way and students had to give their informed consent prior to data collection. Moreover, students could participate in the learning activity without sharing their data for research. This study was approved by the responsible institutional review board (HREC number: 050-2020).

\subsubsection{Baseline Models}
\label{subsec:baseline}
We assessed the performance of our sequential models to more simple baseline models. Random forest (RF) models were successfully used in previous work \cite{cock2021early} to (early) predict students' level of conceptual understanding gained through interacting with an interactive simulation. \cite{cock2021early} experimented with neural network models and RF models with different type of features and did not find significant differences regarding predictive performance of the different model and feature combinations. We selected RF model with \textit{Action Span} features (\texttt{RF}) as a baseline for our experiments, as this encoding is most similar to our action-state sequences. The \textit{Action Span} features can be easily built from our state and action categories. For each time step $m$, the encoding of the triplet $(e'_m, s'_m, d_m)$ is similar to a one-hot encoded vector, where all entries are $0$ except the one representing $e'_m \times s'_m$ (state-action combination), which is equal to $d_m$. We therefore obtain a vector $v_m$ of dimensions $c_s \times c_e$. The raw interaction sequence $R_u$ for student $u\in\mathcal{U}$ then becomes $I_u = \{v_0, ..., v_{\tilde{n}_u\}}$. We flatten $I_u$ by summing all vectors $v_m$, resulting in a vector where each cell represents the amount of time in seconds the student spent doing each type of state-action combination. We then normalise the vector by the total duration of the interaction so that the model does not consider the length of each interaction, but rather the proportion of time spent on each condition.

\subsubsection{Optimisation Protocol}
Both \texttt{GRU} and \texttt{SA-GRU} are relatively sensitive to \textit{seeds} which have an influence on all weight initialisation. To temper the effects of randomness on the models' training, we used a cross validation with seed mitigation to optimise the neural network models. The usual nested cross-validation optimisation protocol was conducted for the baseline RF model. We evaluated performance of all models using the macro-averaged area under the ROC curve (AUC). 

\textbf{Optimisation for RF}. We optimised the \texttt{RF} model using a 10-fold nested cross validation stratified over the labels $L_u$. We use this step as an evaluation mean for the RF and as a basis for parameter optimisation for the GRU-based models. We ran the inner grid search on the following hyperparameters: the \textit{number of decision trees} $[3, 7, 9, 11, 13, 15, 17]$, the \textit{split criterion} $[gini, entropy]$, the \textit{maximum depth} $[5, 7, 9, 11, 13]$, the \textit{minimum samples split} $[3, 5, 7, 9, 11]$.
%\par We start by  conducting a 10-fold \textbf{nested} cross validation stratified across their conceptual understanding (what and how many concepts they grasped after interacting with the simulation) for the three algorithms. We optimise the random forest algorithm from scikit learn \cite{scikit-learn} on the \textit{number of decision trees} [3, 7, 9, 11, 13, 15, 17], the \textit{split criterion} [gini, entropy], the \textit{maximum depth} [5, 7, 9, 11, 13], the \textit{minimum samples split} [3, 5, 7, 9, 11]; the class weights [balanced subsample] and maximum features per base classifiers [automatic] are fixed parameters. 

\textbf{Optimisation for GRU and SA-GRU}. For the two sequential models, we performed initial protoyping using a 10-fold nested cross validation (using the same folds as for the RF model) and a small number of seeds. We trained both the \texttt{GRU} and \texttt{SA-GRU} for $150$ epochs, using a categorical crossentropy loss and an Adam optimiser. We tuned the following hyperparameters: dropout rate after the GRU layer $[0.02, 0.05]$ and the number of cells $[32, 64]$ in the GRU layers. The initial experiments demonstrated that: the selected hyperparameter values in the inner grid search were the same for a majority of the folds, the categorical cross entropy loss on the inner validation data set tended to converge after $20-30$ iterations, and predictive performance of the models seemed to vary depending on the seed. We therefore decided to choose a fixed architecture for the \texttt{GRU} and \texttt{SA-GRU} models and limit the number of epochs to $30$ for all our experiments. For Beer's Law Lab the selected parameters were a dropout rate of $0.02$ and $32$ units for the GRU layer. For the Capacitor Lab, we also use $32$ units in the GRU Layer and a dropout rate of $0.05$. We evaluated the models using 10-fold cross validation (based on the same outer folds as the RF model). To mitigate the potential effects of randomness, we trained both models over $n$ different seeds and averaged predictive performance across seeds. For our experiments on the full state-action sequences (see Sections \ref{sec:resrq1} and  \ref{sec:resrq3}), we used $n=60$ seeds. Since we observed only minor differences in predictive performance across seeds, we reduced the number of seeds to $n=10$ for our early prediction experiments (see Sections \ref{sec:resrq2} and  \ref{sec:resrq3}).

%We optimise the dropout rate for the SA-GRU [0.02, 0.05] as well as the number of GRU cells [32 or 64]. We train both GRU and SA-GRU on seed 193 with 150 epochs without early stopping, using a callback retrieving the model with the best validation score at the end of the 150 epochs. Once the optimal GRU/SA-GRU architecture has been selected, we re-run another gridsearch where the only hyperparameter we change is the seed [0, 16, 60,  3, 64, 69, 75, 96,  5, 77]. Finally, we run the optimal architecture on the optimal seed to compute the test scores for each fold.

%\textbf{Model Evaluation} \par We observe that the chosen sets of parameters in the architecture-gridsearch are often similar, and that the seed selection introduces minor variations across folds. To report fairer results and mitigate the potential effects of randomness, we re-train both models over 60 seeds on the most common selected architecture (from 1 to 60).  We decide to only run each algorithm for 30 epochs without early stopping nor callbacks to retrieve the model with the best validation score at the end. This design decision was based on the categorical cross-entropy loss and roc values measured on the validation sets during the \textit{nested cross validation} training phase: we observed on multiple instances (one of them shown in figure~\ref{fig:trainvalidation}) that the validation scores tended to plateau and not improve after 30 epochs approximately.

%\textbf{Early Predictions} 

\begin{comment}
\begin{figure}
\Description{}  % Alt text
\centering
\includegraphics[width=\columnwidth]{EDM-template/figures/design-decision.png}
\caption{Categorical cross-entropy loss and roc over 150 epochs for a SA-GRU algorithm initialised with seed 1.}
\label{fig:trainvalidation}
\end{figure}
\end{comment}

%%%%%%%%%% Research question 1: Full Sequence, ChemLab %%%%%%%%%%%%%%%%%%%%%
\subsection{RQ1: Full Sequence Prediction}
\label{sec:resrq1}
In a first experiment, we investigated whether our proposed models were able to predict students' level of conceptual understanding based on their interaction data. We used the evaluation data set collected with the Beer's Law Lab simulation to answer RQ1.

\textbf{Predictive Performance}. Figure \ref{fig:chemlabfullpred} illustrates the predictive performance in terms of AUC for the \texttt{GRU}, the \texttt{SA-GRU}, and the \texttt{RF} baseline. Both sequential models outperform the \texttt{RF} baseline: using \texttt{GRU} and \texttt{SA-GRU} models we improve the AUC by $~10\%$ ($AUC_{GRU} = 0.77$, $AUC_{SA-GRU} = 0.76$, $AUC_{RF} = 0.70$). We also observe that the \texttt{RF} model exhibits a higher variability across folds than the two sequential models. For those, the minimum AUC is close to $0.70$ ($AUC_{min,GRU} = 0.69$, $AUC_{min,SA-GRU} = 0.68$). In contrast, performance of the \texttt{RF} model drops below $0.6$ based on the fold ($AUC_{min,RF} = 0.58$). We also performed a preliminary analysis on model bias according to protected attributes. Specifically, we grouped the students based on the available protected attributes and computed predictive performance in terms of AUC separately for the different groups. We found that the \texttt{GRU} model is slightly biased towards male students ($AUC_{m,GRU}=0.78$, $AUC_{f,GRU}=0.73$), while the two other models do not show any gender bias. All models show a bias in terms of region, with a higher AUC for region A ($AUC_{A,GRU}=0.78$, $AUC_{A,SA-GRU}=0.78$,$AUC_{A,RF}=0.76$) than for region B ($AUC_{B,GRU}=0.69$, $AUC_{B,SA-GRU}=0.66$,$AUC_{B,RF}=0.63$).

\begin{figure}[!t]
\Description{AUC of the GRU for the Beer's Law Lab experiment: mean is 0.77, spread is around 0.12. AUC of the SA-GRU model: mean is 0.76, spread is around 0.15. AUC of random fores: mean is 0.7, spread is around 0.3.}
  \centering
  \includesvg[width=0.9\columnwidth]{figures/full-chemlab-bubbleplot.svg}
  \caption{AUC of the GRU, SA-GRU, and RF models on the evaluation data set collected from Beer's Law Lab. Predictions were made based on the complete sequential interaction data of the students.}
  \label{fig:chemlabfullpred}
\end{figure}

\textbf{Attention Interpretation}. While adding self-attention to the GRU does not increase predictive performance of the model (there is no significant difference in the performance of the \texttt{GRU} and \texttt{SA-GRU} model), the self-attention scores enable interpretation of the such black-box models. The heatmap in Fig. \ref{fig:attheatmapfullchemlab} shows the normalised attention scores for the \texttt{SA-GRU} model over $150$ time steps. For each student $u\in\mathcal{U}$, we extracted the output (dimension: $n_u \times f$) of the self-attention layer of the \texttt{SA-GRU} model (see Fig. \ref{fig:sagrudl}) and normalised it to make the attention scores comparable between models. We then averaged across all students. The number of students decreases rapidly with an increasing number of time steps (Fig. \ref{fig:chemlabfullpred} (top)). In fact, for $90\%$ of the students, $n_u \leq 150$.

We observe that the model seems to pay most attention to two of the states (\textit{green-red} and \textit{no absorbance}). The former state, \textit{green-red}, indicates a green laser colour and a red solution colour while the absorbance is measured. As expected, exploring with this parameter setting is important for solving the ranking task. The latter state, \textit{no absorbance}, indicates that the absorbance (outcome variable of the task) was not displayed, which makes solving the task impossible. Also the two other states (\textit{green-green} and \textit{absorbance}) seem to have phases of higher importance over time. For the \textit{no absorbance} state, we can see that the the model seems to pay less attention to it with an increasing number of time steps. Generally, the actual state of the simulation seems to be considered as more important than a specific action of the student. Regarding the action, the model seems to pay attention to state \textit{pdf}, which refers to students checking the task description and hence the configurations to be ranked. Also experimenting with \textit{concentration} and \textit{width} seems to have some importance. Interestingly, the importance of taking a \textit{break} varies over time steps. Finally, the model does not pay attention to the \textit{concentration-lab} action.

\begin{figure}[t]
\Description{histogram representing the number of students having at least x time steps. More people are included up until 10 time steps. There is a first dip at 30 time steps, where around 50 people stop interacting with the simulation. Less than 50 students have at least 150 time steps. Below is a graph showing the attention scores for the different features. The higher scores are for absorbance between 0 and 25 time steps and for the state green red between 10 and 25 time steps.}
  \centering
  \includegraphics[width=\columnwidth]{EDM-template/figures/attention-full-chemlab.png}
  \caption{Normalized attention scores for the SA-GRU over $150$ time steps (bottom). Number of students with $\mathbf{n_u \geq t}$ for $\mathbf{t = 1,...,150}$ (top).}
  \label{fig:attheatmapfullchemlab}
\end{figure}

\textit{In summary, this first experiment demonstrated that our proposed models yielded a $10\%$ increase in AUC over the RF approach suggested in previous work \cite{cock2021early}. Furthermore, the sequential models also exhibit a lower variance across folds. Finally, by adding self-attention to a GRU model, we were able to provide interpretations of what type of student exploration behavior will lead to successfully solving the task.}

%%%%%%%%%%%%%%%%% Research question 2: Early Prediction %%%%%%%%%%%%%%%%%%%%%
% write in paragraphs FP/TP, FN/TN on gender -> assessment on gender bias (with respect to protected attributes), region bias, year bias -> 
% => For LSTM, SSAN, RF (average roc per group over all seeds)
\subsection{RQ2: Early Prediction}
\label{sec:resrq2}
In our second experiments, we were interested in predicting students' level of understanding \textit{during} their interaction with the simulation. We therefore did not use all students' full interaction sequences, but used partial interactions up to a time step $l$ \jade{when the student went over that limit}. Therefore to build the features $F^{l,SA}_u$ for student $u\in\mathcal{U}$, we only used the interactions $I^l_u$ as a basis for building the features (see also Section \ref{sec:featextract}). We trained all our models for $l = 30, 40, 50, 60$. We did not make predictions earlier as we did not expect a model to be able to accurately predict conceptual understanding after only a few student actions. We further limited $l \leq 60$ as the number of students decreases for higher time steps (see also Fig. \ref{fig:attheatmapfullchemlab} (top) \jade{which indicates the amount of remaining students per time step}). At each time step $l$, we made predictions for students with state-actions sequences at each length $l$ (e.g. $\tilde{n}_u \geq l$). For students with shorter sequences (e.g., $\tilde{n}_u < l$), we used the last available prediction. We used the evaluation data set collected with Beer's Law Lab to answer RQ2.

\textbf{Predictive Performance}. Fig. \ref{fig:earlypredchemlab} illustrates the AUC of the different models for early prediction at $t = 30,40,50,60$. We again observe that the \texttt{RF} baseline model performs inferior to the sequential models. It achieves an AUC of $0.59$ after $30$ time steps and manages to only slightly improve over time with an AUC of $0.61$ after $60$ time steps. The AUC of the \texttt{RF} is $0.70$ for full sequence prediction (see Section \ref{sec:resrq1}), we therefore observe a strong increase in predictive performance when observing full sequences. It thus seems that the \texttt{RF} classifiers is not able to extract strong signal from early observations. The use of more elaborate sequential models leads to an up to $15\%$ increase in AUC ($AUC_{30,GRU} = 0.67$, $AUC_{30,SA-GRU} = 0.68$, $AUC_{60,GRU}$ $= 0.72$, $AUC_{60,SA-GRU} = 0.72$). Similar to the full sequences case, \texttt{RF} exhibits a much higher variance across folds than that our proposed models.

\begin{figure}[t]
  \centering
  \Description{Boxplot for the scores of the GRU, SA-GRU and RF at early time steps. The highest mean at time step=30 is for the SA-GRU, right below 0.7. For 40 timesteps, the highest mean is GRU, followed by SA-GRU, both around 0.65, while the mean of the RF is slightly below 0.6. For 50 time steps, SA-GRU performs slightly better than GU, both around 0.7, and the random dorest follows at around 0.65. In all cases, the spread of the boxplot is pretty wide, averaging towards 0.2. }
  \includesvg[width=\columnwidth]{figures/chemlab-early-boxplot.svg}
  \caption{Early predictive performance in terms of AUC for RF, GRU, and SA-GRU for the evaluation data set collected using Beer's Law Lab for $\mathbf{t = 30, 40,...,60}$.}
  \label{fig:earlypredchemlab}
\end{figure}

\textbf{Attention Interpretation}. Next, we investigated whether attention scores differed between an early prediction and a full sequence prediction model, i.e. whether the model paid attention to different features when making early predictions.

Figure \ref{fig:attheatmap30ChemLab} shows the normalised attention scores for the \texttt{SA-GRU} model trained to predict at time step $t=30$ The scores in the heatmap were calculated following the same procedure as for the full sequences case (see Section \ref{sec:resrq1}). Similar to our findings on full sequences, we observe that the states generally seem to be assigned higher scores than the actions. While we again observe that the \textit{no absorbance} and \textit{green-red} states have relatively higher scores, we also observe that these scores vary over time. The scores of the \textit{no absorbance} state clearly decrease over time. This finding might suggest that many students realise during their first $10-15$ interactions with the simulation that the absorbance display should be turned on (by default, transmittance is displayed). In contrast, the scores of the \textit{green-red} state increase over time, indicating that after being able to observe the outcome variable (absorbance), it is important to select the optimal colours for laser (green) and solution (red). For the actions, we observe the same picture as for the full predictions. The \textit{concentration-lab} action gets little attention (it is probably also a rare action), while manipulating \textit{width} and \textit{concentration} gets similar attention over time. Checking the task description is mainly important early on. The model does not pay attention to \textit{break} for the first $10$ time steps. We hypothesise that `thinking' breaks do not occur often during initial interaction when students are still focused on understanding the task and have not yet started their exploration.\\

\begin{figure}[t]
\Description{Attention scores for the SA-GRU which was trained for interactions up until 30 time steps. Most attention is given to the state no absorbance, especially until the 12th time step, where it is above 0.02. Then, it is also given to the green red state from the 12th time step on at a lesser scale (higher than 0.01). }
  \centering
  % [trim=left bottom right top, clip]
  \includegraphics[trim = 0cm 0.7cm 8.5cm 0cm, clip,width=\columnwidth]{EDM-template/figures/attention-early30-chemlab.pdf}
  \caption{Normalised attention scores for SA-GRU trained for predicting at $\mathbf{t = 30}$ time steps for Beer's Law Lab.}
  \label{fig:attheatmap30ChemLab}
\end{figure}

\textit{In summary, our second set of experiments showed that in case of early prediction, the use of a GRU or SA-GRU model leads to even larger performance increases than in case of full sequences. Depending on the time step, we observe improvements in AUC of $15\%$ compared to the RF baseline. Furthermore, the RF again shows high variability with drops in AUC down to $0.50$. We are again able to provide meaningful interpretations of the attention weights, which is a promising basis for targeted intervention.}


% \subsection{RQ3: Transferring to a Different Setting}
\subsection{\jade{RQ3: Generalisation}}
\label{sec:resrq3}
In our last experiment, we were interested in assessing the generalisability of the developed models. While both learning activities were based on a ranking task, the underlying simulation as well as the population are different. We therefore evaluated our models on the transfer data set collected from the Capacitor Lab simulation.

\textbf{Prediction on Full Sequences}. We first evaluated the generalisability of the different model by predicting on the full interaction sequences of the validation data set. Figure \ref{fig:fullpredcap} illustrates the predictive performance in terms of AUC for the \texttt{GRU}, the \texttt{SA-GRU}, and the \texttt{RF} baseline. We observe that all the models achieve a very high AUC for the Capacitor Lab data set. The sequential models achieve an AUC of $0.96$ (\texttt{GRU}) and $0.96$ (\texttt{SA-GRU}) respectively, while the AUC of the \texttt{RF} baseline is $0.95$. Again the \texttt{RF} baseline model shows higher variability, achieving a minimum AUC of $0.86$. For the \texttt{GRU} and \texttt{SA-GRU}
models, we achieved a minimum AUC of $0.9$ and $0.89$ respectively. For Capacitor Lab, we ran the same bias analysis on protected attributes as for Beer's Law Lab, showing that models are not biased with respect to field (the only known protected attribute for this data set).
 
While the \texttt{SA-GRU} model does not outperform the other two models, we again extracted the attention weights of this model and interpreted them. Figure \ref{fig:attheatmapfullcapacitor} shows the normalised attention scores of the \texttt{SA-GRU} models over a $100$ time steps. We chose to limit to $100$ time steps as for $90\%$ of the students $\tilde{n}_u \leq 100$. Again, the scores displayed in the heatmap were calculated using the procedure described in Section \ref{sec:resrq1}. Similar to our findings on Beer's Law Lab, we observe that the states (\textit{stored energy}, \textit{closed circuit}) receive higher attention than the actions. For \textit{stored energy}, attention scores increase up to time step $30$ and then decrease again after time step $60$. We assume that students needed some time to explore the simulation and figure out that the stored energy display needs to be turned on (it is by default turned off in the simulation). For the \textit{closed circuit} state, attention scores decrease over time, but there are always phases of increased activity. In order to be able to solve the ranking task, it is important to experiment with the closed as well as the open circuit, as detected by the model. The model also seems to pay attention to actions related to \textit{voltage}, \textit{plate area}, and \textit{plate separation}, which are the other three components in the simulation that influence the stored energy. Moreover, \textit{breaks} are important for different phases within the sequences. Hence, the model seems to detect when students take a thinking break and considers that as important.

\begin{figure}[!t]
\Description{Capacitor Scores for the GRU, SA-GRU and RF. All models have a mean of around 0.95, with the mean+std equal to 1. }
  \centering
  \includesvg[width=\columnwidth]{figures/full-capacitor-bubbleplot.svg}
  \caption{AUC of the GRU, SA-GRU, and RF models on the validation data set collected from CapacitorLab. Predictions were made based on the full interaction data of the students.}
  \label{fig:fullpredcap}
\end{figure}

\begin{figure}[!t]
\Description{On top is a histogram showing the distribution of the students throughout different time steps. Most people (193) are kept until 20 time steps. At 60 time steps, less than 100 students are still present in the corpus. Most attention is given to the circuit state (0 if closed, 1 if opened): the scores are higher than 0.014 until around 20 time steps, and it is still higher than the other action features than the action features. The second highest attention score is for the stored energy. It goes above 0.008 from 15 time steps on.}
  \centering
  \includegraphics[width=\columnwidth]{EDM-template/figures/attention-full-capacitor.png}
  \caption{Normalized attention scores for CapacitorLab for the SA-GRU over $150$ time steps (bottom). Number of students with $\mathbf{n_u \geq t}$ for $\mathbf{t = 1,...,150}$ (top).}
  \label{fig:attheatmapfullcapacitor}
\end{figure}

\textbf{Early Prediction}. Next, we also trained the different models for early prediction on Capacitor Lab. Figure \ref{fig:earlypredcaplab} shows the AUC of the evaluated models for prediction on $t=30,40,50,60$ time steps. We see that the AUC of the two sequential model is close to $0.80$ already after observing $30$ student interactions ($AUC_{30,GRU} = 0.8$, $AUC_{30,SA-GRU} = 0.81$). Predictive performance of the \texttt{RF} model is slightly lower ($AUC_{30,RF} = 0.76$). After $60$ time steps, all the models achieve an AUC larger than $0.8$ ($AUC_{60,GRU} = 0.9$, $AUC_{60,SA-GRU} = 0.9$, $AUC_{60,RF} = 0.88$). We observe that all three models show a similar variability under this task.

\begin{figure}[!t]
\Description{AUC scores of the capacitor lab for different time steps. The means increase from 0.8 to 0.92 as the time steps increase. All performances are comparable, with the random forest scoring slightly below GRU and SA-GRU. }
  \centering
  \includesvg[width=\columnwidth]{figures/capacitor-early-boxplot.svg}
  \caption{AUC of the GRU, SA-GRU, and RF models for early prediction ($\mathbf{t = 30, 40, ..., 60}$) on Capacitor Lab.}
  \label{fig:earlypredcaplab}
\end{figure}

\textit{In summary, our results demonstrate that the proposed models can be transferred to a different learning environment and population. In case of full interaction data, the performance of the models is inline with the RF baseline, in case of early prediction, the sequential models outperform the baseline. Furthermore, the addition of self-attention again enabled us to identify the key points in the exploration process.}
